Using Flow Specifications of Parameterized Cache Coherence Protocols for Verifying Deadlock Freedom

We consider the problem of verifying deadlock freedom for symmetric cache coherence protocols. In particular, we focus on a specific form of deadlock which is useful for the cache coherence protocol domain and consistent with the internal definition of deadlock in the Murphi model checker: we refer to this deadlock as a system- wide deadlock (s-deadlock). In s-deadlock, the entire system gets blocked and is unable to make any transition. Cache coherence protocols consist of N symmetric cache agents, where N is an unbounded parameter; thus the verification of s-deadlock freedom is naturally a parameterized verification problem. Parametrized verification techniques work by using sound abstractions to reduce the unbounded model to a bounded model. Efficient abstractions which work well for industrial scale protocols typically bound the model by replacing the state of most of the agents by an abstract environment, while keeping just one or two agents as is. However, leveraging such efficient abstractions becomes a challenge for s-deadlock: a violation of s-deadlock is a state in which the transitions of all of the unbounded number of agents cannot occur and so a simple abstraction like the one above will not preserve this violation. In this work we address this challenge by presenting a technique which leverages high-level information about the protocols, in the form of message sequence dia- grams referred to as flows, for constructing invariants that are collectively stronger than s-deadlock. Efficient abstractions can be constructed to verify these invariants. We successfully verify the German and Flash protocols using our technique.

==> FormalModelBackup.tex <==
\section{Protocols, Flows and \MDeadlock Freedom: Background}
\label{sec:formalModel}
\subsection{Preliminaries}

A protocol \Protocol(N) consists of $N$ symmetric cache agents, with
ids from the set $\IndexSet = \{1,2,3,\ldots,N\}$. We follow our prior
approach~\cite{ParamVerMurali} (which was inspired by the approach of
Kristic~\cite{ParamVerifCMPKristic}) in formalizing cache coherence
protocols.

{\em Index Variables:} The protocol uses index variables from the set
\IndexVarSet quantified over the set of index values
$\IndexSet$. Thus, if $i$ is an index variable, then $i$ takes values
from the domain $\IndexSet$.

{\em State Variables:} The state of the protocol consists of local and
global variables, shared between agents. Each of these type of
variables can either hold values from Boolean domain (variables with
values from generic finite domains can be represented as a set of
Boolean variables) or pointers which can hold agent ids. We represent
the Boolean variables in the global state as $G_B$, while the pointers
as $G_P$. The Boolean local state variables of each agent $i$ is
encoded as $L_B[i]$, while the local pointer variables as $L_P[i]$.
The pointer variables, thus, have values from the domain $\IndexSet
\cup \{null\}$, where $null$ represents that the variable does not
hold any index value.

{\em Rules: } The protocol consists of a set of rules written on the
state variables. Each rule $rl(i)$\footnote{We assume that each rule
  consists of one index $i$ for ease of exposition, our method applies
  to rules with more than one index as well.} can be written
as: \[rl(i): rl(i).\rho \rightarrow rl(i).a,\]

where, $i$ is a variable (referred to as {\em index} variable) with
values in \IndexSet, $rl(i)$ is the rule name, $rl(i).p$, the guard,
is a propositional formula on the global variables and local variables
of agent with index value stored in $i$, and $rl(i).a$ is the action
which updates the global variables and local variables of agent with
index value stored in $i$.

{\em Protocol:} A {\em protocol} is a state transition system
$(S,\Theta,T)$, where $S$ is the set of protocol states, $\Theta$ the
initial states of the protocol, and $T \subseteq S \times S$ is the
transition relation described using a set of rules. The protocol state
$s$, then, is a valuation of the variables in $V_S$ and $V_L[i]$, for
all $i$. Thus, there is a transition $\tau(i_v)$ from state $s$ to
$s'$ if there is a rule $rl(i)$ and value of index variable $i=i_v$,
s.t. $rl(i_v).\rho$ holds in $s$, and $s'$ is obtained by applying
$rl(i_v).a$ to $s$. In state $s$, we say that the rule $rl(i)$ is {\em
  enabled} (for agent $i_v$) if the guard $rl(i_v).\rho$ is $true$.
When the enabled transition $\tau(i_v)$ is executed, we say that the
rule $rl(i)$ is {\em fired} for agent $i_v$.

{\em Note:} The protocol is symmetric since the set of local variables
for each agent is identical, and the rules, $rl(i)$ can be
instantiated for each agent as well. 

{\em Protocol execution:} We assume interleaving semantics for the
protocol, i.e., at any state $s$, any of the enabled rules can fire
and when a rule is fired, its action is applied to update the state
atomically. An execution trace of the protocol from a state $s_0$ to a
state $s_n$ with $n$ transitions in between looks as follows: $s_0
\rightarrow^{\tau_0} \rightarrow^{\tau_1} \rightarrow^{\tau_2} \ldots
\rightarrow^{\tau_{n-1}} s_n$.

\nop{
%{\em Protocol Transitions and messages model}
{\em Transitions:} The transitions of the protocol are indexed over
$i$, \(\tau_1(i),\tau_2(i),\tau_3(i) \ldots \tau_k(i)\). In this
paper, we express the state transitions of the protocol using {\em
  rules} (we use the words rule and transition interchangeably). A
rule $rl(i)$ is a guard-action pair which is written as $rl(i).\rho
\Rightarrow rl(i).a$, where the guard $rl(i).\rho$ (also referred to
as $\rho(i)$ for brevity) is a Boolean expression on variables in
$V_L[i]$ and $V_S$, and the action $rl(i).a$ (also referred to as
$a(i)$ for brevity) is an update to variables in $V_L[i]$ and
$V_S$. We say that a rule is {\em enabled} in a state $s$ if its guard
$\rho$ evaluates to $true$ in $s$, else the rule is {\em disabled}. An
enabled rule is said to have fired when it applies its action $a$ to
update the state. When a rule fires, the corresponding transition
occurs.
}

\subsubsection{\MDeadlock Definition}
We define a protocol state $s$ to be a {\em \mdeadlock state} if no rule
in that state is enabled. Then a protocol is \mdeadlock free if in all
states, there exists at least one transition which is enabled. This
can be expressed as the invariant:

\[\bigvee_{i} \bigvee_{rl(i)} rl(i).\rho,\] 

i.e., the disjunction of guards of all rules of all agents $i$ must be
$true$ in all reachable states.

%deadlocks if at some point
%in future, a state with all guards $false$ is reachable. Formally,
%deadlock freedom then, can be expressed as a temporal formula \[ \lnot
%F G(\forall i: \bigwedge_{rl(i)} \lnot rl(i).\rho),\] where, $F$ is
%the {\em eventually} operator and $G$ the {\em always} operator of
%temporal logic.


%A deadlock state, then, is a state in which
%$\g(P_T)$

\subsubsection{Flows}
Flows describe the basic organization of rules for implementing the
high-level requests in a protocol (for example a request for \Shared
or \Exclusive access or an \Invalidate). We model a flow $fl(i)$ as a
set of rules of the form $\{$$rl_1(i), rl_2(i), \ldots rl_n(i)$$\}$
which accomplish a high-level request\footnote{For ease of exposition
  we assume that the guard and action of a rule are over the variables
  of a single agent. Thus, a flow containing such rules also involves
  a single agent. In general, a rule and thus a flow can involve a
  larger but fixed number of interacting agents as well. Our approach
  can easily be generalized to that case.}.  These rules are ordered,
i.e., for rule $rl_k(i)$ to fire, all rules before that in the flow
must have already been fired. Then, given an execution trace, flows
naturally induce an ordering condition on the trace s.t. a rule
$rl_k(i)$ can fire only if all rules $rl_1(i) \ldots rl_{k-1}(i)$ have
fired.  Formally, we denote this by $rl_k(i).pre^{fl}$ which holds on
a trace if the rules preceding $rl_k(i)$ have all fired.

A protocol essentially then consists of a set of flows $fl_1, fl_2,
fl_3, \ldots, fl_k$. In order to process a high-level request, a
protocol may use a combination of flows. As an example, in order to
execute a request for exclusive access, the German protocol uses the
\Exclusive and \Invalidate flows.

\subsubsection{Some definitions:}
Given a set of transitions $T$, the operator $\g(T)$ is $true$ if at
least one transition in the set of transitions $T$ must be enabled,
else it is $false$. Thus, it is a disjunction of the guards of
transitions in $T$.  Then, we say an agent $i$ is enabled if at least
one of its rules is enabled, i.e., $\g(i)$ holds.  Next, we say that a
flow is enabled if at least one of its rules is enabled, i.e.,
$\g(fl(i))$ holds.  

Finally, in case a flow $fl(i)$ is not enabled, we say it is {\em
  blocked} on rule $rl(i)$ if the precondition of the rule
$rl(i).pre^{fl}$ holds but the guard of the rule $rl(i).\rho$ is
$false$.

\subsection{German Protocol Implementation}
\nop{The German protocol implements 3 high-level requests: (1) an
\Exclusive request initiated by an agent for getting a read or a write
permission (agent state with read and write permission is denoted by
$E$), (2) a \Shared request for getting a read only permission (agent
state denoted by $S$), and (3) an \Invalidate request initiated by the
directory to take away all the permissions from an agent (agent state
with no permissions is denoted by $I$).
}
%\subsubsection{Relevant Global Variables}
%The directory points to the cache whose request is currently being
%served (for a particular cache line) using the pointer
%\curptr. Further, it stores the request type from \curptr in
%\curcmd. Next, \exgntd is set to true if some cache has exclusive
%access, else it is set to false. Finally, a set of variables, \shrset,
%stores the caches which share a particular cache line. Thus,
%\shrset[i] is true if cache $i$ has a copy of the line. Finally, an
%auxiliary variable $cache\_inv$ (FIX: not shown in code) points to
%some cache $c$ such that \shrset[c] is true---$cache\_inv$ is null if
%and only if \shrset is false for all caches.

%\subsubsection{Relevant Local Variables}

%\subsubsection{German Protocol Implementation}
The German protocol consists of agents which can have \Exclusive
($E$), \Shared ($S$) or \Invalid ($I$) access to a cache line: the
agents request these access rights by sending messages to a shared
directory. The directory is modeled as a set of global variables. The
directory serves one agent at a time: it stores the id of the agent
being served in the variable $CurPtr$. It also stores the nature of
request in the variable $CurCmd$ with values in $\{ReqE,ReqS,Empty\}$,
where $ReqE$ represents a request for \Exclusive access, $ReqS$ for
\Shared and $Empty$ for no request. Finally, the directory tracks if
\Exclusive access is granted to some agent or not using the variable
$ExGntd$: it is $true$ if access is granted and $false$ otherwise.
The code for the implementation of the \Exclusive request is shown in
\Fig{Fig:ExclusiveCode}\footnote{For increasing clarity, compared to
  the original code presented in Appendix~\ref{AppendixGermaCode},
  some variable names have been changed as well as some details not
  relevant to the discussion have been skipped. Note that variable
  names start with capital letters for the sake of consistency with
  the original code.}.

\input{flowCode.tex}

In processing the \Exclusive request, before sending the grant
$SendGntE(i)$, the directory checks if there are any sharers (by
checking $ShrSet$ = $\{\}$). If there are sharers, the \Invalidate
flow is invoked for each agent in $ShrSet$.  Upon invalidation of all
agents in $ShrSet$, the $ShrSet$ becomes empty and so the
$SendGntE(i)$ rule becomes enabled for execution.

We show the code for the $SendInv(i)$ rule below. (The complete code
of the protocol is provided in the Appendix~\ref{AppendixGermaCode}
for the interested reader.)  We denote the condition for invoking
\Invalidate (i.e. enabling the first rule of the \Invalidate flow
$SendInv(i)$) by $Inv\_Cond \land (ShrSet \neq null)$, where,
\(Inv\_Cond: CurCmd = ReqE \lor (CurCmd=ReqS \land ExGntd=true)\) can
be identified from the guard of the rule $SendInv(i)$.

\vspace{.3cm}
\begin{minipage}{\textwidth}
\footnotesize
\Ruleset{$\forall$ i : \IndexSet;}{SendInv(i)}{InvChannel[i].cmd =
  Empty $\land$ i $\in$ ShrSet $\land$ InvSent[i] = false 

\hspace*{.4cm}  $\land $ ((CurCmd = ReqE) $\lor$ (CurCmd = ReqS $\land$ ExGntd =
  true))}{InvChannel[i].cmd = Inv; InvSent[i] = true;}
\end{minipage} 

\nop{
The German protocol models a directory as a set of global variables.
The directory stores the index value of the agent whose request is
currently being served in a global variable $CurPtr$ with values in
$\{\{null\} \cup [1,N]\}$. $CurPtr=i$ if request of agent $i$ is being
served and $CurPtr=null$ if no request is being served. Next,
information about the current request being served by the directory is
encoded in the variable $CurCmd$ with values in $\{ReqE,ReqS,Empty\}$,
where $ReqE$ represents a request for \Exclusive access, $ReqS$ for
\Shared access and $Empty$ for no request. The directory also
maintains a list of agents which share a particular cache line,
denoted by $ShrSet$. Finally, the directory tracks if \Exclusive
access is granted to some agent or not using the Boolean variable
$ExGntd$: it is $true$ if access is granted and $false$ otherwise.

Each agent $i$ stores its current status in local variable
$Cache[i].State$ with values in ${I,S,E}$, where $I$, $S$ and $E$
stand for $Invalid$, $Shared$ and $Exclusive$, respectively. Next, the
agents and directory communicate with each other through channels: the
implementation of the German protocol uses separate channels for
separate requests. Agent $i$ sends requests for \Shared or \Exclusive
access to the directory on $ReqChannel[i]$. The directory in turn
sends grants to agent $i$ using the channel $GntChannel[i]$.  Finally,
the directory sends \Invalidate to agents through the channel
$InvChannel[i]$: in order to track that an \Invalidate request is sent
to a particular agent $i$, it keeps a variable $InvSent[i]$ which is
$true$ if the request has been sent and $false$ otherwise.

\input{flowCode.tex}

%The code snippet implementing the Exclusive request for the German
%protocol is shown in \Fig{Fig:ExclusiveCode}. 
\paragraph{Code for \Exclusive request}
\Fig{Fig:ExclusiveCode} shows the relevant code details\footnote{For
  increasing clarity, compared to the original code presented in
  Appendix~\ref{AppendixGermaCode}, some variable names have been
  changed as well as some details not relevant to the discussion have
  been skipped. Note that variable names start with capital letters
  for the sake of consistency with the original code.} for the
implementations of the $SendReqE(i)$, $RecvReqE(i)$, $SendGntE(i)$ and
$RecvGntE(i)$ rules of the \Exclusive flow (flow shown in
\Fig{figGermanFlowsExcl}). Notice that the guard of the rule
$SendGntE(i)$ checks if there are no sharers of the cache line
($ShrSet$ = $\{\}$). Rest of the guards and actions of the rules in
the figure are self-explanatory.

\paragraph{Code for \Invalidate request}
For the implementation of the \Invalidate request (flow shown in
\Fig{figGermanFlowsInv}), for the sake of brevity, we only provide the
code for the rule $SendInv(i)$ which implements an \Invalidate request
initiated by the directory for a sharer:
% This is shown in \Fig{fig:codeSendInv}.

\vspace{.3cm}
\begin{minipage}{.3\textwidth}
\footnotesize
\Ruleset{$\forall$ i : \IndexSet;}{SendInv(i)}{InvChannel[i].cmd =
  Empty $\land$ i $\in$ ShrSet $\land$ InvSent[i] = false 

\hspace*{.4cm}  $\land $ ((CurCmd = ReqE) $\lor$ (CurCmd = ReqS $\land$ ExGntd =
  true))}{InvChannel[i].cmd = Inv; InvSent[i] = true;}
\end{minipage} \vspace{.2cm}

The guard of this rule checks the following two key conditions: (1)
first, it checks if the current request for \Shared or \Exclusive
access requires the directory to initiate an \Invalidate request to
the agents sharing the cache line. This is true when the current
request is either for an \Exclusive access or, is for a \Shared access
with another agent already having an \Exclusive access. This is stated
as the condition: \(Inv\_Cond: CurCmd = ReqE \lor (CurCmd=ReqS \land
ExGntd=true).\) (2) And second, it checks whether there is an agent
$i$ which needs to be invalidated, by checking $(i \in ShrSet)$.
%This is done by checking the condition ($(invChannel[i].cmd
%= empty)$ $\land$ $(i \in ShrSet$) $\land$ $(InvSent[i] = false)$).
}
\nop{
This rule checks if the channel for sending invalidates
($invChannel[i]$) is empty, that $i$ is in the set of sharers
($ShrSet$), that invalidate has not yet been sent (tracked using
$invSet[i] = false$) and that the current request is either exclusive
or it is for shared but some other cache has exclusive access
(i.e. $((CurCmd = ReqE)$ $\lor$ $((CurCmd = ReqS)$ $\land$ $(ExGntd =
true)))$, denoted by $invCond$).
}

\nop{


The protocol code snippets implementing the Exclusive and Invalidate
requests for the German protocol are shown in \Fig{Fig:ExclusiveFlow}
and \Fig{Fig:InvalidateFlow} respectively\footnote{The complete code
  is in the appendix.}.  


\subsubsection{Flows}
The German protocol consists of three flows: \Exclusive flow, \Shared
flow and \Invalidate flow. The \Exclusive flow processes a request for
write access, \Shared for read access and the \Invalidate flow for
invalidating some cache. The \Invalidate flow is a sub-flow of \Shared
and \Exclusive flows. These flows are detailed as follows:

%shown in \Fig{figGermanFlows} can be
%written as 
\begin{itemize}
\item{\Exclusive:} {\bf ReqExclusive(i)}: $SendReqE(i)$, $RecvReqE(i)$,
  $SendGntE(i)$, $RecvGntE(i)$.

\item{\Shared:} {\bf ReqShared(i)}: $SendReqS(i)$, $RecvReqS(i)$,
$SendGntS(i)$, $RecvGntS(i)$.

\item{\Invalidate:} {\bf SendInval(i)}: $SendInv(i)$, $SendInvAck(i)$,
  $RecvInvAck(i)$.
\end{itemize}

\subsubsection{Protocol Code}
The code snippets for the Exclusive and Invalidate flows of the German
protocol is presented in Murphi language~\cite{} in
\Fig{Fig:ExclusiveFlow} and \Fig{Fig:InvalidateFlow}
respectively\footnote{The complete code is in the appendix.}.  These
code snippets, along with global state are explained below.

%\Fig{figGermanCode} (courtesy~\cite{CMP}).

\nop{
\paragraph{Murphi Syntax:} Murphi language consists of {\em rulesets} 
which is a collection of {\em rules}, where each rule is a guarded
action. For example, $SendReqS$ is a ruleset which represents a set of
rules $1..N$, where rule $i$ (denoted by $SendReqS[i]$) corresponds to
$i^{th}$ cache sending a request for shared access. The guard of
$SendReqS[i]$ is $Chan1[i].Cmd = Empty \land Cache[i].State = S$ and
the action is $Chan1[i].Cmd := ReqS$.  {\em Observe that each message
  in the flows shown above correspond to a ruleset in the code.}

\paragraph{Murphi Semantics:} Each rule is executed atomically. Thus, at any time, 
Murphi non-deterministically selects a rule which has its guard true
and executes it.
}

\paragraph{Relevant Global State:} The directory points to the cache
whose request is currently being served (for a particular cache line)
using the pointer \curptr. Further, it stores the request type from
\curptr in \curcmd. Next, \exgntd is set to $true$ if some cache has
exclusive access, else it is set to false. Finally, a set of
variables, \shrset, stores the caches which share a particular cache
line. Thus, \shrset[i] is true if cache $i$ has a copy of the
line. Finally, an auxiliary variable $cache\_inv$ (FIX: not shown in
code) points to some cache $c$ such that \shrset[c] is
true---$cache\_inv$ is null if and only if \shrset is false for all
caches.

\paragraph{Code for Exclusive access}

\paragraph{Code for Invalidate access}

%\begin{figure}
%\hspace*{-5cm} \includegraphics[scale=1]{./Figures/germanProtocol.pdf}
%\caption{German Protocol}
%\label{figGermanCode}
%\end{figure}

\input{flowCode.tex}



\nop{
The flows for the German protocol are shown in
\Fig{figGermanFlows}. These flows represent the order in which various
messages in the protocol are passed, in order to accomplish a high
level request. Thus, they provide high level information about the
protocol. The German protocol consists of the following flows:

\begin{itemize}
\item \Shared: The \Shared flow, shown in \Fig{figGermanFlowsShrd}
  processes a request from cache $i$ for shared access. It consists of
  messages \{$sendReqS$, $RecvReqS$, $SendGntS$, $RecvGntS$\} passed
  between the requesting cache and directory.

\item \Exclusive: Similar to shared flow, shown in
  \Fig{figGermanFlowsExcl}.

\item \Invalidate: The \Invalidate flow is a sub-flow of \Shared and
  \Exclusive flows: it has rules \{$sendInv$, $sendInvAck$,
  $recvInvAck$\}. It is present in both figures,
  \Fig{figGermanFlowsShrd} and \Fig{figGermanFlowsExcl}.
\end{itemize}
}
}


==> Introduction_Backup.tex <==
\section{Introduction}
Verification of deadlock freedom for message passing protocols, such
as cache coherence protocols, is an important practical problem. Such
protocols involve an arbitrary number of symmetric, interacting agents
(e.g. caches). Thus, they are candidates for parameterized
verification techniques. While parameterized techniques for safety
properties have seen considerable success in verifying key properties
like mutual exclusion (i.e. no two caches have write permissions to a
cache line simultaneously) for industrial scale cache coherence
protocols~\cite{DeadlockFlash, CMP, ParamVerifMuraliIndust}, their
success in verifying deadlock freedom has been limited. In this work
we focus on enabling direct application of such state of the art
parameterized techniques for proving deadlock freedom as well.

\subsection{Characterizing Deadlock for Protocols}
We model a protocol as a parameterized state transition system
\Protocol(N) which consists of \(N\) symmetric agents, where $N$ is a
finite but unbounded parameter, along with some global state shared
between the agents. The agents have ids $1,2,3,\ldots,N$: each agent
$i$ has transitions \(\tau_1(i),\tau_2(i),\tau_3(i) \ldots
\tau_k(i)\). Each transition $\tau_j(i)$ is modeled as a guard-action
pair. A transition is {\em enabled} if its guard is $true$, else it is
{\em disabled}. When an enabled transition occurs, its action is
applied to update the state.

A protocol implements high-level requests, for example a request for
read or write permissions for a cache coherence protocol. Then, the
ultimate goal of any deadlock (or livelock) verification effort is to
prove that each high-level request eventually gets a response.
%: i.e. response
%properties of the form $G(req \rightarrow F(res))$, where $req$ is the
%request, $res$ the response, and $G$ and $F$ are the $always$ and
%$eventually$ operators of temporal logic. 
However, such a property is a liveness property. While there is
existing work in parameterized verification of liveness
properties~\cite{CounterAbstraction, Baukus:02a, InvisibleRanking,
  McMillanLiveness}, these approaches typically have limited
scalability due to complex abstractions required for verifying
liveness. Further, direct verification of liveness is hard due to
limited support from existing model checking
tools~\cite{DeadlockSayak}.

\nop{
A protocol implements high-level requests, for example a request for
read or write permissions for a cache coherence protocol. Then, the


a protocol can be informally understood as a state transition system
which implements high-level requests (e.g. requests for read write
permissions in a cache coherence protocol). Each transition of this
system is represented as a guard-action pair. A transition is {\em
  enabled} if its guard is $true$, else it is {\em disabled}.


A protocol is a parameterized state transition system \Protocol(N),
with $N$ symmetric agents, where $N$ is a finite but unbounded
parameter.  Informally, the protocol consists of states with
transitions $\tau$, where the transition $\tau$ has a guard $\tau.g$
and an action $\tau.a$ which updates the state. A transition $\tau$ is
{\em enabled} in a state $s$ if its guard $\tau.g$ is $true$ in $s$,
else it is {\em disabled}.

A protocol implements high-level requests, for example a request for
read or write permissions for a cache coherence protocol. Then, t

For such a system, the ultimate goal of any deadlock (or livelock)
verification effort is to prove that each high-level request
eventually gets a response.
%: i.e. response
%properties of the form $G(req \rightarrow F(res))$, where $req$ is the
%request, $res$ the response, and $G$ and $F$ are the $always$ and
%$eventually$ operators of temporal logic. 
However, such a property is a liveness property---while there is
existing work in parameterized verification of liveness
properties~\cite{CounterAbstraction, DeadlockWSIS,
  InvisibleRanking, McMillanLiveness}, these approaches typically
either have limited scalability due to complex abstractions required
for liveness or tend to be largely manual. Further, direct
verification of liveness is hard due to limited support from existing
model checking tools~\cite{DeadlockSayak}.
}

An alternate approach towards verifying response properties is to
analyze causes for failure of the property. Two key causes for the
failure of liveness properties are: (1) an unfair scheduler, i.e. a
request never gets a chance to get served, or (2) a lack of response
to a request due to the protocol getting stuck in a deadlock or
livelock. There are multiple formal definitions of deadlock in
literature (see for example \cite{DeadlockClassic, DeadlockBingham,
  xmasVmcai, DeadlockSayak}): we define a deadlock state as one where
the protocol gets completely blocked, i.e., a deadlock state is a
state in which all its transitions are disabled. Correspondingly, we
define a livelock as a loop of one or more states in which, once a
protocol gets stuck, no high-level requests get served.  Assuming
fairness, deadlock typically is a more commonly observed cause for
failures of response properties for industrial protocols compared to
livelock~\cite{DeadlockBingham}.
%---proving deadlock freedom
%is the focus of this work. 
%In this paper we focus on
%proving deadlock freedom, by verifying a stronger property derived
%using high level information in the form of {\em flows}, as described
%in \Sec{sec:flows}.

\subsection{Challenges in Proving Deadlock Freedom}
The main complexity in deadlock verification is that a deadlock
witness can involve an arbitrary number of agents deadlocked in a
classical resource dependency cycle~\cite{DeadlockClassic}---unlike
say mutual exclusion where a witness for the violation involves the
state of the two caches with erroneous write permissions.  Formally,
mutual exclusion can be specified on a protocol model as an invariant
of the form $\forall i,j:\phi(i,j)$, where $\phi$ is a propositional
logic formula with two index variables $i$ and $j$ stating that agents
$i$ and $j$ cannot have simultaneous write permissions.  Invariants
of this form involve a small number (say $k$) of universally
quantified index variables and thus can be verified using efficient
abstractions like the standard data type
reduction~\cite{ConcDSDataTypeRed}. This abstraction keeps just $k$
agents and abstracts away the state of all the other agents, replacing
them with a stateless environment.  The usage of data type reduction
along with state of the art parameterized techniques has been
instrumental in successful verification of industrial scale
protocols~\cite{DeadlockFlash, CMP, ParamVerifMuraliIndust}.

However, unlike mutual exclusion, specification of deadlock freedom as
an invariant with a small number of indices is challenging: since a
deadlock violation can involve an arbitrary number of agents, its
specification $\phi$ must in general be indexed over an arbitrary
number of agents.  In this work we address this by leveraging
high-level information to specify invariants involving a small number
of quantified index variables. These invariants collectively imply
deadlock freedom and can be directly verified using data type
reduction and existing parameterized verification techniques.

\subsection{Proving Deadlock Freedom using Flow Properties}
\label{sec:flows}
\subsubsection{Flows}
%Protocols implement high level requests, for example, cache coherence
%protocols implement requests for read/write permissions. This
%implementation is done by processing a request through a set of
%messages (or transitions)---
{\em Flows} provide information about the messages passed in the
protocol implementation for processing high-level requests.  These are
readily available in industrial documents in the form of charts and
tables. In this work we show how these can be used for proving
deadlock freedom.

As an example, the German protocol consists of \{\Exclusive, \Shared,
\Invalidate\} flows, for processing \Exclusive, \Shared, and
\Invalidate requests. \Fig{figGermanFlows} shows the \Exclusive and
\Invalidate flows for the German protocol.
%These show the set
%and ordering of messages passed in the implementation in order to
%process an exclusive request. 
Thus, for example, in order to implement the \Exclusive request, the
messages $SendReqE(i)$, $RecvReqE(i)$, $SendGntE(i)$ and $RecvGntE(i)$
are passed between the agent $i$ and the directory, as shown
\Fig{figGermanFlowsExcl}.

The messages passed in the protocol implementation are modeled as
transitions and thus have guards and actions. For example,
$SendGntE(i)$ has a guard
%$SendGntE.g$ 
checking that the set of caches with read access, i.e. $ShrSet$, must
be empty and an action which sends a message to cache $i$ granting a
write access.  We say that a flow is {\em enabled} if one of its
messages has a guard which is $true$.

%\begin{figure}
%  \includegraphics[scale=0.5]{./Figures/germanExcl.jpg}
%\caption{German protocol flows}
%\label{figGermanFlows}
%\vspace{-0.75cm}
%\end{figure}

\begin{figure}
\centering
\hspace*{- 0.75cm}
\subfloat[\Exclusive flow]{
\label{figGermanFlowsExcl}
  \includegraphics[scale=.65]{./Figures/germanExcl.jpg}
}
\hspace*{1.75cm}
\subfloat[\Invalidate flow]
{
\label{figGermanFlowsInv}
  \includegraphics[scale=.65]{./Figures/germanInv.jpg}
}
\caption{Flows for the German protocol.}
\label{figGermanFlows}
\end{figure}

\subsubsection{Specifying Flow Properties for Deadlock Freedom}
Since in a deadlock state, there are no enabled transitions, the
guards of all transitions 
%$\tau$ 
are $false$. Thus, a protocol is deadlock free if at all times, there
is at least some enabled transition in the protocol. We leverage flows
to prove this and verify that at all times there is at least one flow
which is enabled.  
%This in turn implies that some guard of some
%transition of that flow is enabled at all times.
%Since flows provide high level
%information about how transitions are organized to implement high
%level requests, showing some flow is enabled at all times is easy.
%we show
%some transition is enabled at all times by showing that some flow is
%enabled at all times.

Formally, we show the flow property referred to as \Enabled: ``at all
times, there exists {\em some} flow which is enabled''. In temporal
logic, this property can be stated as $G(\exists fl(i): \g(fl(i))$,
where $G$ is the $always$ operator of temporal logic, $fl(i)$ a flow
at agent $i$, and $\g(fl(i))$ is the disjunction of guards of all the
transitions in $fl(i)$. For example for the German protocol,
%flow, one can write
%$g$(\Exclusive($i$)) as $sendReqE(i).g$ $\lor$ $RecvReqE(i).g$ $\lor$
%$SendGntE(i).g$ $\lor$ $RecvGntE(i).g$ and thus 
the \Enabled property can be written as $G(\exists fl(i):\g(fl(i)))$,
where $fl(i)$ $\in$ $\{$\Exclusive($i$), \Invalidate($i$),
\Shared($i$)$\}$.

In order to verify the \Enabled property, the existential quantifier
needs to be eliminated.  This is accomplished by the user by adding
witness variables which store the index of the
%information (i.e. skolemization) about which agent has an
agent which must have some flow enabled, for a set of states of the
protocol (specified using a predicate on state
variables)~\footnote{This process can be understood as skolemization
  for an Invariant with an existential quantifier.}. As an example,
for the German protocol, two of the invariants obtained on adding
witness variables are as follows: (1) the \Exclusive flow is enabled
for a set of states where there are no sharers of the cache line,
i.e., $(\SetOfSharers=\{\})$ $\rightarrow$ $\forall i:
\g(\Exclusive(i))$, and (2) for the set of states where there are
sharers, the \Invalidate flow must be enabled for a sharer, i.e.,
$\lnot (\SetOfSharers = \{\})$ $\rightarrow$
$\g(\Invalidate(Sharer))$, where, $Sharer$ is a witness variable
pointing to a sharer of the cache line.

\subsection{Parameterized Verification of Flow Properties}
As can be seen from the German protocol example, the invariants
generated on iteratively adding witness variables for the enabled
flows involve a small number of index variables (equal to the maximum
number of agents involved in sending or receiving messages in a
flow). Then, these can be verified for an arbitrary number of agents
by direct application of standard data type
reduction~\cite{ConcDSDataTypeRed} along with state of the art
parameterized verification techniques. We use the CMP (CoMPositional)
method~\cite{DeadlockFlash,CMP}: this method is an
abstraction-refinement based method which, along with data type
reduction, has seen considerable success in verifying safety
properties of industrial scale protocols. The final experimental flow
is shown in \Fig{figExperimentalSetup}.

%n tandem with data type reduction to verify the
%\Enabled property---
%The CMP method is an abstraction-refinement based method which, along
%with data type reduction, is one of the most successful industrial
%approaches used for verifying safety properties of industrial scale
%protocols~\cite{ParamVerifMuraliIndust}. 
%The final experimental flow is shown in \Fig{figExperimentalSetup}.

%\subsection{Experimental Flow}
%Bla

\begin{figure}
\centering
\hspace*{-0.5cm}  \includegraphics[scale=.6]{./Figures/progressSpecGenBigPict.jpg}
\caption{Experimental Flow}
\label{figExperimentalSetup}
\end{figure}


\subsection{Key Contributions}
We make the following key contributions:

%get around this issue by leveraging the following key properties:
\begin{itemize}
\item We show how high-level information can be leveraged to specify
  and then iteratively generate a set of invariants by adding witness
  variables pointing to enabled flows. These invariants are amenable
  to industrial scale parameterized verification techniques. (Section
  3)

\item We show how the \Enabled property implies deadlock
  freedom. (Section 3)

\nop{
present a method which enables the user to specify if some
  flow is enabled (i.e. the \Enabled property) as a set of invariants,
  by leveraging high-level information (flows).
}

\item Finally, we evaluate the utility of our approach by verifying
  the Flash and German protocols for an arbitrary number of
  caches. (Section 5)
\end{itemize}

\subsubsection{Key Limitation: }
The key limitation of our approach is that the specification has to be
generated manually through iteratively inspecting counterexamples,
identifying witness variables, and splitting invariants. This can
potentially be automated if the information about the witness
variables is available in the flow diagrams (and it is in certain
cases). However, we believe that adding the information iteratively on
inspecting the counterexample is easier on the user, instead of
requiring this information a-priori in the flow diagrams. Further, the
number of iterations required to add this information for even complex
protocols like Flash were observed to be small (3 for the Flash
protocol).

\subsection{Relevant Related Work}
Bingham et al.~\cite{DeadlockBingham, DeadlockBinghamCAV}
parametrically verify deadlock freedom as a safety property and can
handle complex protocols such as the Flash protocol. Like ours, their
approach is based on the CMP method as well. In particular, their
method extends the CMP method to handle formal proofs for deadlocks:
their notion of deadlock is to specify it by using user identified
Quiescent states, i.e. a state in which no resources are held. They
specify a state to be deadlock free if a Quiescent state is reachable
from it. In order to accomplish formal proofs of deadlock freedom,
they extend the CMP method by using a combination of abstractions
(also referred to as {\em mixed}
abstraction~\cite{mixedAbstractions}): (1) an over-abstraction for the
set of reachable states and (2) an under-abstraction of the path from
a reachable state to a Quiescent state. Both these abstractions have
to be manually tuned in order to prove deadlock freedom. While their
approach is manual like ours, we believe that flows provide a more
natural way of thinking about protocols and specifying
properties. Further, our approach uses well understood
over-abstractions which are easier than coming up with quiescent
states and then tuning over and under abstractions manually.

Among parameterized techniques for verifying liveness (and thus
response properties), Macmillan has verified liveness properties of
FLASH protocol parametrically~\cite{DeadlockFlash,
  McMillanLiveness}---their proof works on the basis of lemmas and
fairness assumptions supplied to the model checker. In contrast, our
work leverages high-level information for specifying and verifying
deadlock: this helps in reducing manual effort. Baukus et al. verified
liveness properties of the German protocol~\cite{Baukus:02a} using
their logic WS1S.  However, the complexity of WS1S is
super-exponential, thus restricting scalability.  Fang et al. provide
another interesting approach for verifying liveness: they use
invisible ranking~\cite{InvisibleRanking} (they used counter
abstraction~\cite{CounterAbstraction} in prior work). Their approach
involves using ranking functions for constructing abstractions to
verify liveness of algorithms like the Szymanski’s and Bakery
algorithms.
%Since our approach verifies
%deadlock instead of end-end response properties These approaches either
%tend to have limited scalability or require increased manual effort:
%since our works focuses just on deadlock instead of end-end response
%properties, we are able to scale to large protocols with reduced
%manual effort.
%The usage of ranking
%functions adds state the abstraction, thus limiting scalability.

%or using
%counter-abstraction~\cite{LivenessCounterAbstraction}.
%Apart
%from Macmillan's flash work, no other liveness verification approach
%scales to Flash protocol[check].

%The state of the art in industry is to formally verify deadlock
%freedom for a small number of caches or to do simulation based
%verification.  Both these approaches are incomplete[CHECK].

Next, the concept of detecting deadlock (and livelock) by reducing
them to a set of invariants (e.g. progress invariants) is well known
(see for example~\cite{xmasVmcai, DeadlockSayak}). Our approach is
similar to these: we also seek to reduce deadlock freedom to a set of
invariants. However, our approach leverages flows in order to reduce
deadlock verification to a set of invariants which then can readily be
used with state of the art techniques. Further, these flows along with
the CMP method are already used in industry for designing and
verifying complex protocols~\cite{ParamVerMurali}: thus they are a
promising approach for verifying deadlock freedom as well.

\nop{Further, the usage of the CMP method in our approach helps in
  achieving scalability to complex protocols like Flash---which seems
  unlikely for the approaches for network protocols.  } \nop{ These
  approaches work with user identifying a set of primitives to model a
  system, or a set of progress assumptions [Explain], or bla bla bla.
  This work handles verifying deadlock freedom for complex control
  logic by first modeling it using a fixed set of primitives and then
  reducing it to a set of invariants. Our work is similar in spirit to
  these---however to the best of our knowledge there is no existing
  work for verifying deadlock freedom for protocols which leverages
  the existing flow documents.  The usage of flows drastically
  simplifies the effort required in coming up with witness
  variables. Further, none of these techniques work with the CMP
  method, and thus have no chance of scaling.
%we
%focus on parameterized systems which are not amenable to modeling
%using known primitives.
}

Finally, among parameterized verification techniques for protocols,
there are numerous existing techniques in literature apart from the
CMP method. Some examples include Invisible Invariants for
safety~\cite{InvisibleInvariants}, Counter Abstraction for
safety~\cite{CounterAbstraction}, Indexed
predicates~\cite{IndexedPredicates}, ordinary model
checking~\cite{Abdullah:99a}, WS1S~\cite{Baukus:02a},
learning~\cite{Grinchtein:06} and strengthening split
invariants~\cite{Cohen:07}. Further, a transaction-based
method~\cite{ParkDill:96} and a predicate abstraction-based
method~\cite{DasDill:99} were also used to verify cache coherence
protocols. However, these techniques either do not scale to larger
protocols or tend to require increased manual effort to scale to
larger protocols. The demonstrated success of the CMP method along
with the data type reduction abstraction for industrial scale
protocols motivated us to use it in our approach.


==> Introduction_backup26Aprl.tex <==
\section{Introduction}
We verify deadlock freedom for symmetric cache coherence protocols.
Consider a cache coherence protocol \Protocol(N) where the parameter
\(N\) represents an unbounded number of (cache) agents. The protocol
implements requests sent by the agents using messages exchanged in the
protocol. As a protocol designer, the holy grail for verification is
the request-response property: i.e. every request from an agent
eventually gets a response. Since this is a liveness property and hard
for existing model checking tools, designers then resort to verifying
simpler properties such as deadlock freedom to identify causes for
response property failure. 

The literature is abundant with various definitions of
deadlock~\cite{}: we verify for deadlock errors in which the entire
protocol gets stuck, i.e., no agent of the protocol can make any
transition. We refer to such failures as maximal deadlock
(\mdeadlock): this kind of failures, while weaker than other broader
classes of deadlock failures, is commonly observed in industry and is
consistent with the internal definition for deadlock used by the
Murphi model checker as well~\cite{}. 

Since an \mdeadlock error involves all the agents getting stuck and
unable to make any transition, verification of \mdeadlock freedom
naturally is a parameterized verification problem. Parameterized
verification techniques work by using sound abstractions to reduce the
unbounded model to a finite model that preserves the property of
interest. These abstractions typically tend to be simple
over-abstractions which keep a small number of agents ($1$ or $2$) as
is and replace all the other agents with an abstract environment: such
abstractions have had considerable success in verifying key safety
properties like mutual exclusion and coherence even for industrial
scale protocols~\cite{CMP, ParamVerifMuraliIndust, ParamVerMurali}.
%Each agent has an id from
%the set \IndexSet = \{1,2,3.\ldots,N\} \(i\) be \(\tau_1(i) \ldots
%\tau_t(i)\) (each transition $\tau$ is a guard-action pair with guard
%$\tau.g$ and action $\tau.a$.). 

While successful for properties like mutual exclusion and coherence,
the application of such abstractions for parameterized verification of
properties like \mdeadlock gets challenging. This is because an
\mdeadlock error involves all of the arbitrarily large number of
agents getting stuck and unable to make progress: simple
over-abstractions like above will not preserve this error since they
discard state of most of the agents.
%Authors in a prior paper, in fact,
%had to resort to mixed abstractions (i.e. a combination of under and
%over abstractions) to verify deadlock
%freedom~\cite{DeadlockBingham}. 
In this paper we show how high-level information about these protocols
can be leveraged to construct invariants which are collectively
stronger than the \mdeadlock property. These invariants are amenable
to efficient abstractions like data type reduction which have been
used in the past in verifying industrial scale protocols.
%Our method leverages high-level information about the
%protocol present in the form of {\em flows}, as described through the
%example below.

\subsection{Deadlock in the German Protocol}
The German protocol is a popular benchmark for existing protocol
verification work in literature~\cite{DeadlockBingham, CMP}. The
protocol implements high-level requests for \Exclusive, \Shared, and
\Invalidate access to a cache line.

Architects informally describe protocols using special diagrams,
referred to as {\em flows}. These provide information about the
messages passed in the protocol implementation for processing
high-level requests. Flows are readily available in industrial
documents in the form of charts and tables. 

\Fig{figGermanFlows} shows the \Exclusive and \Invalidate flows for
the German protocol. Thus, for example, the \Exclusive request from
agent (cache) $i$ to the directory is implemented as follows: the
message (transition) $SendReqE(i)$ is sent by the agent $i$ to the
directory. The directory receives this message and updates its
book-keeping state ($RecvReqE(i)$).  Next, if the directory is able to
grant a right for exclusive access, it sends the message $SendGntE(i)$
to agent $i$.  The agent $i$ receives this grant ($RecvGntE(i)$) and
transitions to \Exclusive state. These messages are passed (in that
order) between the agent $i$ and the directory, as shown
\Fig{figGermanFlowsExcl}.

\begin{figure}
\centering
\hspace*{- 0.75cm}
\subfloat[\Exclusive flow]{
\label{figGermanFlowsExcl}
  \includegraphics[scale=.65]{./Figures/germanExcl.jpg}
}
\hspace*{1.75cm}
\subfloat[\Invalidate flow]
{
\label{figGermanFlowsInv}
  \includegraphics[scale=.65]{./Figures/germanInv.jpg}
}
\caption{Flows for the German protocol.}
\label{figGermanFlows}
\end{figure}

Next, it may be noted that the message $SendGntE(i)$ is sent only if
no other agent has \Shared access to the cache line. In case another
agent, say $j$, has access to the cache line, the directory uses the
\Invalidate(j) flow to first invalidate $j$. This flow proceeds by the
directory sending the invalidate ($SendInv(j)$), the agent $j$ sending
the acknowledgment ($SendInvAck(i)$), and the directory receiving it
($RecvInvAck(i)$).

\subsubsection{Deadlock Situation:} Now consider the case when the 
acknowledgment (ack) sent by the agent $j$ gets dropped. In this case,
the directory is blocked and waiting on the $ack$. The blockage of
directory leads to all the $N$ agents in the protocol getting blocked
as well. Thus no transition in the protocol is enabled. In a realistic
implementation of the protocol, one would assume the directory would
timeout if the $ack$ is not received: even in that case, this kind of
a bug would negatively impact the performance of the protocol.

In this paper, we check for freedom against a class of deadlock errors
where the entire protocol gets blocked, i.e., all the agents are
stuck. In order to express this mathematically, we model the agents of
the protocol \Protocol(N) to have transitions such that each
transition $\tau$ has a guard $\tau.g$, which is $false$ if the
transition can not happen.  Thus, the protocol is stuck if the guards
of all the transitions are false, i.e., \(\bigvee_{\tau} \tau.g.\)

\subsection{Challenge in verifying deadlock}
The key challenge in verifying the above property is that it is a
disjunction of all the guards of the parametrized protocol. Thus, a
violation of the above property will be a state in which all the
guards are false, i.e., when \(\bigwedge_{\tau} \lnot \tau.g\)
holds. However, this violation will in high likelihood be masked by
any over-abstraction due to the extra transitions added in the
over-abstraction process.

One approach to address the above issue is to use a combination of
over and under abstractions (i.e. a mixed abstraction), as described
in a prior deadlock verification work~\cite{DeadlockBingham}. While
very promising in verifying an important class of deadlock properties,
while believe the use of mixed abstraction is fairly complex and
effort intensive. 

\subsection{Key Insight}
%The key problem with the deadlock property is that it involves a
%disjunction of all the guards, which is not amenable to abstraction.
Our method tries to partition the state of the protocol such that in
each partition it can point to an agent $i$ and claim that one of its
transitions must be enabled. This is done by starting with an initial
guess of state partition for which agent $i$ must have an enabled
transition.  In case the agent does not have any transition enabled,
typically there is a particular flow of the agent which is 'stuck'
because the protocol is processing a flow of another agent $j$. This
information is used to refine the partition. This way, we derive
invariants of the form: \(pred \rightarrow \phi(i)\), where $pred$ is
a predicate on protocol state and $\phi(i)$ is a disjunction of
transitions for agent $i$. Invariants of this form are much easier to
check using existing parameterized verification techniques.

\subsection{Key Contributions}
Our method proves deadlock freedom for parameterized protocols
(formalized in \Sec{sec:formalModel}). It works by first generating a
set of invariants which collectively imply deadlock freedom
(\Sec{sec:SpecMethod}). These generated invariants use just one index
(i.e. of the form $\forall i: \phi(i)$) and thus are amenable to state
of the art abstraction techniques, for verification for an unbounded
number of agents (\Sec{sec:CMP}). \Fig{figExperimentalSetup} shows the
setup for our method, and highlights the key contribution of this
paper: generation of invariants collectively implying deadlock freedom
by leveraging high-level information present in $flows$. We verified
two challenging protocols, the German and Flash protocols, using our
method (\Sec{sec:Experiments}).

\begin{figure}
\centering
\hspace*{-0.5cm}  \includegraphics[scale=.5]{./Figures/progressSpecGenBigPict.jpg}
\caption{Experimental Flow}
\label{figExperimentalSetup}
\end{figure}

\nop{
We make the following key contributions:

%get around this issue by leveraging the following key properties:
\begin{itemize}

\item We show how deadlock freedom verification can be done without
  developing any special techniques by just using existing techniques
  for parameterized verification.

\item We show how high-level information can be leveraged to
  iteratively specify a set of small-indexed invariants that
  cumulatively imply deadlock freedom.

\item Using this method we have verified deadlock freedom of German
  and Flash cache coherence protocls, two well known academic
  protocols.

\end{itemize}
}

\nop{Whenever
the predicate of a subgroup holds on a protocol state, our invariants
show that one of the transitions in the subgroup associated with that
predicate holds.  {\em The key insight is that each subgroup has
  transitions from a small number of agents (1 or 2) and this
  drastically simplifies checking if some transition in that subgroup
  is enabled.}

The partitioning is done by iteratively splitting an initial guess invariant
This results in invariants of the form:

\begin{tabular}{c}

\(cond_1(i) \Rightarrow en_1(i)\) \\
\(cond_2(i) \Rightarrow en_2(i)\)\\
\( \ldots\)\\
\(cond_c(i) \Rightarrow en_c(i)\)

\end{tabular}

\subsection{Experiment, Contributions, limitations}

We model a protocol as a parameterized state transition system
\Protocol(N) which consists of \(N\) symmetric agents, where $N$ is a
finite but unbounded parameter, along with some global state shared
between the agents. The agents have ids $1,2,3,\ldots,N$ and have
local state. The transitions of the protocol are modeled as
guard-action pairs with transitions for processing the requests of
agent $i$ referred to as \(\tau_1(i),\tau_2(i),\tau_3(i) \ldots
\tau_k(i)~\footnote{The indexed transitions may be transitions of
  either the agent or the global state. As an example for a cache
  coherence protocol, these can be the local transitions of cache $i$
  or the transitions of the global directory processing requests of
  cache $i$.}.\) We assume symmetry in transitions.

%%. The guards and actions of the transitions
%%typically refer to the local variables of one (or more) agent $i$:
%%thus a transition \(\tau(i)\) refers to the local state of agent $i$
%%and potentially the global state. We assume symmetry in transitions.
%,\tau_2(i),\tau_3(i) \ldots \tau_k(i)\)~\footnote{The
%  transitions of the directory refer to index of agent and so are
%  clubbed with agent transitions.}. 
%A transition is {\em enabled} if its guard is $true$, else it is {\em
%  disabled}. When an enabled transition occurs, its action is applied
%to update the state.

We define a state to be a deadlock state if no outgoing transitions
are enabled in that state. Then, in order to prove deadlock freedom,
one needs to show that in all reachable states, at least some
transition is enabled. Doing this parametrically for an arbitrary
number of agents is hard, as compared to properties like mutual
exclusion (i.e. no two caches are in Exclusive state simultaneously).

\nop{
Moreover, any attempts to abstract behaviors of agents is counter
productive as this merely adds more transitions, thus further
obfuscating the check that all transitions in original protocol are
blocked.
}

The key difference between safety properties like mutual exclusion and
deadlock freedom is that the counterexamples to the former involve a
small number of agents whereas counterexamples to the latter may
involve all the agents of the system. More precisely, for a
parametrized system \Protocol(N) with \(N\) symmetric agents, mutual
exclusion or coherence can be expressed as a two-index property

\[\forall i, j \in [1..N]. \phi(i,j).\]

A counterexample to this will involve exactly two agents, 1 and 2 (by
symmetry). This allows us to construct finite abstractions focusing on
a small number of agents (2 in this case) that can be efficiently
model checked~\cite{CMP,ParamVerMurali, ParamVerifMuraliIndust}. On
the other hand, \emph{a counterexample to deadlock freedom may involve
  all the agents of the system.}  Abstracting away agents will lead to
the deadlock being missed. Thus efficient abstractions like data type
reduction~\cite{ConcDSDataTypeRed}, which are crucial in successful
verification of mutual exclusion for industrial strength
protocols~\cite{CMP, ParamVerifMuraliIndust, ParamVerMurali}, are not
directly applicable to deadlock freedom.

\subsection{Our Approach}
What we need is an effective way to reduce the unbounded parametrized
problem of verifying deadlock freedom to a finite problem amenable to
model checking. Instead of directly tackling deadlock freedom, our
method enables the user to construct a series of two indexed
properties (invariants) that collectively are stronger than deadlock
freedom.
 
Deadlock freedom can be specified as an existential assertion: at
every state \(s\) there exists some transition \(\tau_j(i)\) which is
enabled. Formally, this can be written as \[AG \exists i,
\tau_j. (\tau_j(i) \mbox{ is enabled}).\] In order to prove this
property, the existential quantification needs to be eliminated for
the parametrized system. This can be accomplished by identifying for
every state \(s\) the exact transition or set of transitions that have
to be enabled (i.e. skolemization). However, this is hard to
accomplish in general as (1) the exact set of transitions which may be
enabled at any state may be large and involve an arbitrary number of
indices, and (2) enumerating all states is a challenge.

\nop{the system (local
and global state) is parametrized and enumerating all the states and
then identifying transitions will lead to a huge blowup.
}

Our method addresses the above challenges---typically a protocol in
any state is processing a high-level transaction and this can be
leveraged in identifying a subset of transitions which must be
enabled. Our method works by identifying a set of transitions by
leveraging this high-level information such that at least one of these
transitions must be enabled when the high-level transaction is being
processed. Next, instead of enumerating all states, our method enables
the user to derive simple predicates on the protocol, such that these
can be used to refer to a set of states which have a common set of
enabled transitions.

More specifically, message passing protocols are structured around a
series of logical high-level transactions, called
\emph{Flows}~\cite{ParamVerMurali}---flows represent a series of
transitions such that they happen in the order specified and together
they accomplish one logical transaction of the protocol.  As an
example, the German cache coherence protocol consists of \{\Exclusive,
\Shared, \Invalidate\} flows as shown in \Fig{figGermanFlows}. As the
names indicate, these deal with processing the \Exclusive, \Shared,
and \Invalidate access requests. Since a flow represents transitions
for one transaction which involves one or two agents interacting with
the global state, the transitions of the flow are typically on a small
number (one or two) of agents: invariants constructed from these
involve only a small number of agents.

%%Thus, each flow,
%%\(fl(i,j)\)~\footnote{For this paper, we assume flows are on two
%% agents.} represents a set of transitions on agents $i$ and $j$.
%the set of transitions \(\tau_1(i), \ldots,
%\tau_t(i)\) are grouped into a set of Flows \(fl_1(i), \ldots,
%fl_f(i)\).

Our method enables the user to derive invariants which are as follows:

\nop{
Our method depends crucially on the fact that dealing with Flows
instead of transitions allows to easily specify which Flow \(fl\) must
be enabled, that is one of the transitions appearing in it is enabled,
under a given condition.  Our strategy then is to come up with a
series of properties
}

\begin{tabular}{c}

\(cond_1(i) \Rightarrow en_1(i)\) \\
\(cond_2(i) \Rightarrow en_2(i)\)\\
\( \ldots\)\\
\(cond_c(i) \Rightarrow en_c(i)\)

\end{tabular}

Here, $en_p(i)$ is a subset of enabled transitions (typically a
disjunction of the guards of the transitions of all the flows
involving the agent $i$) when the condition $cond_p(i)$
holds. Further, it is trivial to identify for which agent $i$
$cond_p(i)$ holds. As an example, for cache coherence protocols,
$cond_p(i)$ checks if a global pointer at the directory points to the
cache $i$ when the directory is processing a request of that
cache. Further, $en_p(i)$ can be generated as a disjunction of the
guards of the transitions of the flows involved in processing requests
from cache $i$.


\begin{figure}
\centering
\hspace*{- 0.75cm}
\subfloat[\Exclusive flow]{
\label{figGermanFlowsExcl}
  \includegraphics[scale=.65]{./Figures/germanExcl.jpg}
}
\hspace*{1.75cm}
\subfloat[\Invalidate flow]
{
\label{figGermanFlowsInv}
  \includegraphics[scale=.65]{./Figures/germanInv.jpg}
}
\caption{German protocol flows}
\label{figGermanFlows}
\end{figure}


Note that the above set of \emph{Flow invariants} are all universally
quantified properties with a small number of indices. Thus, they can
be checked using existing parametrized techniques. In this work, we
use the CMP method~\cite{ParamVerMurali,CMP} to verify these
invariants.

\nop{In fact, in the style of CMP method, the \emph{Flow
  invariants} can be generated on iteratively starting from an initial
guess. Once we have a set of invariants we can try to verify them. If
the proof goes through we are done. Otherwise, the counter example
will led us to split the \(cond_1,..,cond_c\) leading to more
conditions. Since parameterized verification is undecidable in general
this process doesn't have to terminate always but in practice
protocols are well-behaved and the proof either terminates or we find
a real counter example, see~\ref{sec:experiments}.
}

\begin{figure}
\centering
\hspace*{-0.5cm}  \includegraphics[scale=.5]{./Figures/progressSpecGenBigPict.jpg}
\caption{Experimental Flow}
\label{figExperimentalSetup}
\end{figure}


We make the following key contributions:

%get around this issue by leveraging the following key properties:
\begin{itemize}

\item We show how deadlock freedom verification can be done without
  developing any special techniques by just using existing techniques
  for parameterized verification.

\item We show how high-level information can be leveraged to
  iteratively specify a set of small-indexed invariants that
  cumulatively imply deadlock freedom.

\item Using this method we have verified deadlock freedom of German
  and Flash cache coherence protocls, two well known academic
  protocols.

\end{itemize}

\nop{ The rest of the paper is organized as follows. In the next
  section, we formalize the notions already presented here. In
  Section~\ref{example}, we demonstrate the method in action by using
  the German cache coherence protocol as an example. In
  Section~\ref{CMP}, we describe the CMP method and present the
  overall method. Section 5 presents our experimental results and
  Section 6 concludes the paper.  }

\nop{
\subsubsection{Key Limitation}
The key limitation of our approach is that the specification has to be
generated manually through iteratively inspecting counterexamples,
identifying witness variables, and splitting invariants. This can be
automated if the information about the witness variables is available
in the flow diagrams (and it is in certain cases). However, we believe
that adding the information iteratively on inspecting the
counterexample is easier on the user, instead of requiring this
information a-priori in the flow diagrams.
}
}


\subsection{Relevant Related Work}

While there are many techniques for verification of standard safety
property, deadlock freedom and liveness in general are not handled as often.
Of the existing techniques, the notables are as follows. Macmillan has
verified liveness properties of FLASH protocol
parameterically~\cite{DeadlockFlash, McMillanLiveness}. The proof works on
the basis of manually supplied lemmas and fairness assumptions. Next, Baukus
et al. verified liveness properties of the German
protocol~\cite{DeadlockWSIS} using a specialized logic called WSIS. However,
the complexity of WSIS is super-exponential, thus the method is not very
scalable.  Fang et al. used counter abstraction to verify liveness
properties~\cite{LivenessCounterAbstraction}: however the scalability of
counter abstraction is limited as well. Another method by the same group
includes~\cite{InvisibleRanking} to parametrically verify liveness
properties.


Bingham et al.~\cite{DeadlockBingham, DeadlockBinghamCAV} formally
verify deadlock as a safety property for protocols by specifying it
using user identified Quiescent states (i.e. a state in which no
resources are held): they specify a state to be deadlock free if a
Quiescent state is reachable from it. In order to accomplish formal
proofs of deadlock freedom, they require a combination of abstractions
(also referred to as {\em mixed}
abstraction~\cite{mixedAbstractions}): (1) an over-abstraction for the
set of reachable states and (2) an under-abstraction of the path from
a reachable state to a Quiescent state. Both these abstractions have
to be manually tuned in order to prove deadlock freedom. Using their
approach, they successfully verified Flash and German protocols.
While their approach is manual like ours, we believe that flows
provide a more natural way of thinking about protocols and thus
specifying properties using them is easier than coming up with
quiescent states and tuning mixed abstractions manually.

In contrast to all the methods above, our method doesn't develop any
new model checking algorithms for handling deadlock freedom. It
instead strengthens deadlock freedom to a set of universally
quantified small-indexed safety properties which can be verified using
standard techniques. In a loose sense, our approach to strengthening
deadlock freedom verification is similar in spirit to the approach in
the Xmas framework~\cite{xmasVmcai, DeadlockSayak} used for generating
invariants for proving progress properties. 

Finally, among parameterized verification techniques, apart from the
CMP (CoMPositional) method~\cite{CMP}, there are numerous other
techniques for verifying safety properties. Some examples include
Invisible Invariants for safety~\cite{InvisibleInvariants}, counter
abstraction for safety~\cite{CounterAbstraction}, Indexed
predicates~\cite{IndexedPredicates}. The CMP method is a highly
successful parameterized verification technique, numerous work has
been done in the area of parameterized verification, for
e.g.~\cite{InvisibleInvariants, CounterAbstraction,
  IndexedPredicates}. While some of these classical methods are
potentially applicable to concurrent data structures as well, given
the success of the CMP method in verifying industrial cache coherence
protocols~\cite{ParamVerifMuraliIndust}, we believe that our method,
which has a similar flavor to the CMP method, provides a scalable and
effective alternative approach.



==> Makefile <==
FNAME=deadlockPaper
LATEX=latex -src-specials
PDFLATEX=pdflatex

.PHONY : dvi ps pdf clean

pdf : $(FNAME).pdf
ps : $(FNAME).ps
dvi : $(FNAME).dvi

$(FNAME).pdf: $(FNAME).tex *.tex *.bib
	$(PDFLATEX) $(FNAME)
	bibtex $(FNAME)
	$(PDFLATEX) $(FNAME)
	$(PDFLATEX) $(FNAME)
#	/Applications/Adobe\ Reader.app/Contents/MacOS/AdobeReader $(FNAME).pdf &
#	xpdf $(FNAME).pdf &

#$(FNAME).pdf: $(FNAME).ps
#	ps2pdfwr $(FNAME).ps

xpdf:
	xpdf $(FNAME).pdf &

$(FNAME).ps: $(FNAME).dvi
	dvips -t letter $(FNAME).dvi

$(FNAME).dvi: $(FNAME).tex *.tex *.bib
	$(LATEX) $(FNAME)
	bibtex $(FNAME)
	$(LATEX) $(FNAME)
	$(LATEX) $(FNAME)

#	dvipdf $(FNAME).dvi
#	xpdf/acroread $(FNAME).pdf

#$(FNAME).pdf: 	$(FNAME).ps
#	ps2pdf $(FNAME).ps
#	acroread $(FNAME).ps

view:
	xpdf $(FNAME).pdf &

clean:
	rm -f $(FNAME).ps $(FNAME).pdf $(FNAME).dvi $(FNAME).log $(FNAME).aux $(FNAME).blg $(FNAME).bbl
	rm *~
#
#
#(defun james-latex-mode-hook ()
#  (add-to-list 'TeX-command-list
#               '("make pdf" "make %s.pdf" TeX-run-LaTeX nil t)))
#(add-hook 'LaTeX-mode-hook 'james-latex-mode-hook)


==> RelatedWork.tex <==
\section{Related Work}
Parameterized verification

Deadlock verification for Caches

Reduction of liveness to safety

Other liveness verification techniques.

Lot of work has been done in deadlock verification. The reduction of
progress to a bunch of safety properties is not
new~\cite{DeadlockSayak}.


==> SpecMethodBackup.tex <==
\section{Deriving Invariants for Proving \MDeadlock Freedom}
\label{sec:SpecMethod}
In this section, we show how invariants can be derived from flows
which collectively imply \mdeadlock freedom.  At a high-level, our
method works by partitioning the global state of the protocol using
predicates, such that for each partition, some agent $i$ has at least
one transition enabled. Each invariant $inv$ is of the form $inv.pred
\rightarrow \forall i \in \ISet{inv} \, \g(i)$, where $inv.pred$ is a
predicate on the global variables of the protocol, $\ISet{inv}
\subseteq \IndexSet$ s.t. $\lnot(\ISet{inv}=\{\})$~\footnote{This is
  discharged as a separate assertion for model checking.} and $\g(i)$
is a disjunction of the guards of agent $i$. {\em The key insight is
  that since $\g(i)$ has transitions from a single agent, model
  checking $inv$ for an unbounded number of agents is drastically
  simpler than checking the original \mdeadlock property, as discussed
  in \Sec{sec:CMP}.}

Our method works by iteratively model checking invariant $inv$ and on
failure, refining the invariant into two invariants by splitting the
predicate and updating the set $\ISet{inv}$ for each. Suppose, an
invariant of the form $inv.pred \rightarrow \forall i \in \ISet{inv} \,
\g(i)$ fails on model checking. Then, there exists some agent $i_f$
such that when $inv.pred$ holds, $i_f \in \ISet{inv}$ holds and
$\g(i_f)$ is \false. Then, this agent has a flow $fl$ which is blocked
(i.e. it has a rule which is expected to be enabled and so has
precondition \true, however has its guard \false). This blocked flow
is typically waiting for another flow $fl'$ on another agent $i_s$ to
complete. As an example, for German protocol, the \Exclusive flow may
be blocked for agent $i_f$ with the rule $SendGntE(i_f)$ having
precondition \true but guard \false. In this case, it is waiting for
an \Invalidate request to complete for another agent $i_f$, which is
in the set $Sharers$.

The user identifies a global witness variable $\ptr$ which points to
$i_s$, along with a conflict condition $conf$ on the global state
which indicates when $i_s$ is enabled and $i_f$ fails. The user
accomplishes this by using the heuristic that typically, if the rule
$rl$ of flow $fl$ of agent $i_f$ is blocked, $conf$ can be derived by
inspecting the guard of $rl$: $conf$ is the cause for falsification of
$rl.g$.  Further, $\ptr$ identifies the succeeding flow $i_s$; this
can be an auxiliary variable or a state variable already being used by
the protocol. For example, for German protocol, $conf$ can be derived
from the guard of $SendGntE$ and $\ptr$ points to some sharer of the
cache line which is being invalidated.

Using $conf$ and $\ptr$, the invariant can be split into two
invariants. (1) The first invariant excludes the case when conflict
happens from the original invariant, i.e., $inv1: inv.pred \land \lnot
conf \rightarrow \forall i \in \ISet{inv1} \, \g(i)$, where
$\ISet{inv1} = \ISet{inv}$. (2) The second invariant shows that when a
conflict happens, the agent pointed to by \ptr must be enabled and so
the protocol is still \mdeadlock-free, i.e., $conf \rightarrow \forall
i \in \ISet{conf} \, \g(i)$, where $\ISet{conf} = \{i: i \in \IndexSet
\land i=\ptr\}$. For both the invariants, assertions which check that
the corresponding set of indices is not null are also added for model
checking. For example, for $inv1$, this assertion is $inv.pred \land
\lnot conf \rightarrow \ISet{inv1}$.

Our method derives these invariants by iteratively model checking on a
small number of $c$ ($3$ for German protocol) agents. (Once the
invariants are generated on $c$ agents, they are generalized to an
unbounded number of agents, as shown is \Sec{sec:CMP}.) This number
$c$ needs to be chosen such that the proof of \mdeadlock freedom is
expected to generalize to unbounded number of agents: as a heuristic
we found that $c$ should be one more than the maximum number of agents
involved in processing a high-level request. As an example, an
exclusive request may involve two agents, a requesting agent $i$ and
an agent $j$ getting invalidated, so we chose $c$ to be equal to 3.

\nop{
The method starts with a broad enough predicate for each agent and
based on iterative model checking and user analysis of conflicting
flows in the counter-example, this predicate is iteratively split into
smaller predicates. The model checking is done iteratively on a
protocol with a small number $c$ of agents ($2$-$3$). (Once the
invariants are generated on $c$ agents, they are generalized to an
unbounded number of agents, as shown is Sec().) This number $c$ needs
to be chosen such that the proof generalizes easily to unbounded
number of agents: as a heuristic we found that $c$ should be one more
than the maximum number of agents involved in processing any
high-level request to accommodate all possible conflicts among flows.
}

\Fig{fig:MethodOverview} shows the details of the method. Our method
starts with an initial broad guess invariant, $\true \rightarrow
\forall i \in \IndexSet: \g(i)$ (line 1). This states that in all
reachable states, every agent has at least one transition enabled. As
this invariant is \false, this broad guess invariant is refined into
finer invariants, using the loop (lines 2-13). On finishing, the user
is able to derive a set of invariants, $\InvSet$, which collectively
imply \mdeadlock freedom. Further, the user is also able to derive an
assertion set, $\AssertSet$, such that for each invariant $inv$ in
$\InvSet$, an assertion in $\AssertSet$ checks if the set of
indices $\ISet{inv}$ is non-empty when $inv.pred$ holds.

\nop{
The user inspects the returned counter-example (line 5). Unless a
discrepancy between the protocol and the flow is exposed (in which
case the loop exits and the flow/protocol is fixed), the user
identifies the failing agent $i_f$. This agent has a flow $fl$ which
is blocked (i.e. it has a rule with precondition \true but the guard
\false). The blocked flow is typically waiting for another flow
($fl'$) on another agent ($i_s$) to complete (e.g. an \Invalidate
request). The user identifies a global witness variable $\ptr$ which
points to $i_s$, along with a conflict condition $conf$ on the global
state which indicates when $i_s$ is enabled and $i_f$ fails. {\em This
  is essential for generalizing from the counter-example to come up
  with a finer predicate.} Using $conf$ and $\ptr$, the invariants are
updated (lines 11-13).

One heuristic for coming up with $\ptr$ and $conf$ is that, typically,
the flow $fl$ of agent $i_f$ is blocked due to a missing resource-like
variable (e.g. $\lnot (CurPtr=i)$ can be interpreted as $CurPtr$ not held by
$i$). Thus, if the next rule for $fl$ which should be fired is $rl$,
then we observed that $conf$ can be derived by inspecting the guard of
$rl$: $conf$ is the cause for falsification of $rl.g$. Further, $\ptr$
identifies the succeeding flow $i_s$; this can be an auxiliary
variable or at times is a state variable already being used by the
protocol (e.g. $\ptr$ is $CurPtr$).
}

\input{splitMethod.tex}

%% \nop{
%% The invariants of this form are derived iteratively by starting from
%% an initial invariant stating that each agent has some transition

%% guess of a large set of
%% enabled transitions (derived using flows), enabled for all states. In
%% each step, the set of invariants \InvSet is model checked over $c$
%% agents. There are the following possibilities:

%% (1) In case the model passes the invariants, we have generated a set
%% of invariants collectively implying deadlock freedom for $c$
%% agents. These invariants can the be checked for an unbounded number of
%% agents, as discussed in Section 4.

%% (2) In case there is a counter-example and the failing invariant is
%% $inv$, the user inspects the counter-example and the following 3
%% possibilities occur:

%% a) The predicate of the invariant $inv$ is too weak for the set of
%% transitions $inv.\phi$. This occurs when transitions with index $i$
%% cannot be enabled in some state included in $inv.pred$ and instead
%% transitions from some flow of another agent $j$ not included in
%% $inv.\phi$ are enabled. We refer to this case by saying that the flow
%% of agent $i$ is in {\em conflict} with flow of agent $j$.

%% In case of a conflict, the invariant is split to accommodate the
%% conflicting agent by: (1) finding a witness variable $\ptr$ in the
%% protocol which points to $j$ along with the conflicting request $req$
%% and (2) finding a conflict condition $conf$ which must hold when the
%% conflict happens. Then, as shown in \Fig{fig:SplitMethod}, the
%% invariant $inv$ is split to $inv1$ and $inv2$: $inv1$ essentially
%% strengthens the predicate of $inv$ with $\lnot conf$ to remove the
%% conflicting trace, and $inv2$ handles the conflicting case by checking
%% for $\g(req_{\ptr})$ when $conf$ holds. In order to ensure that $\ptr$
%% is not $null$ when $inv2$ holds, we require that $conf \rightarrow
%% \lnot(\ptr=null)$.

%% \input{splitMethod.tex}

%% b) The set of enabled transitions in $inv.\phi$ is too small. This
%% happens if transitions from some flow for the same agent (pointed to
%% by the witness variable) are not included in $inv.\phi$. In this case,
%% the $inv.\phi$ can be simply expanded to include these missed out
%% transitions---since these transitions are on the same witness
%% variable, $inv.pred$ need not be modified.

%% c) One of the flows used in deriving $inv.\phi$ does not match the
%% Murphi model. In this case the user fixes the flows or the Murphi
%% model accordingly.

%% \Fig{figSpecGenDetails} presents the overview of our method for
%% generating the set of invariants $\InvSet$ by iteratively adding
%% witness variables

%% \begin{figure}
%% \includegraphics[scale=.5]{./Figures/progressSpecGenDetails.jpg}
%% \caption{Method Overview}
%% \label{figSpecGenDetails}
%% \end{figure}
%% }
%% \nop{

%% \subsection{Method Details}

%% \subsubsection{Initial Guess Invariant}
%% Since the protocols in this paper implement high-level requests for
%% \Exclusive and \Shared access, we define a set of transitions $S_{ES}$
%% which is essentially the union of transitions of the \Shared and
%% \Exclusive flows. Thus, for the German protocol example, $S_{ES} =
%% fl_{Shared} \cup fl_{Exclusive}$. Then, the initial invariant is
%% essentially $true \rightarrow S_{ES}$.

%% \subsubsection{Refinement by Splitting Invariants}
%% \Fig{figSpecGenDetails} presents the overview of our method for
%% generating the set of invariants $\InvSet$ by iteratively adding
%% witness variables. As shown in the figure, our method starts with an
%% initial set of invariants, $\InvSet$ $=$ $\{true$ $\rightarrow$
%% $\forall i: \g(S_{ES})\}$. Next, the set of invariants, $\InvSet$, is
%% iteratively verified to refine the set of invariants in $\InvSet$. 
%% \nop{The
%% verification is done by model checking a protocol model with a small
%% number of ($c$) agents: as a heuristic this number is one more than
%% the maximum number of agents involved in the guard and action of the
%% rules of the flows of the protocol. Thus, for the German protocol
%% example, $c$ is 2.
%% }

%% \nop{
%% In this section we first show how the \Enabled property can
%% iteratively be reduced to a set of invariants \InvSet by adding
%% witness variables. Next, we provide a proof of soundness of our
%% method, i.e., we show how these generated invariants imply the
%% \Enabled property, which in turn implies deadlock freedom.

%% %The end goal of skolemizing the \Enabled property is to reduce it to a
%% %set of invariants, $\InvSet$. 
%% Intuitively, each invariant in $\InvSet$ provides a witness to a
%% single or a set of agents which have some flow enabled, for a set of
%% states of the protocol. Thus, in our method, we assume that each
%% invariant $inv \in \InvSet$ is of the form $inv.pred \rightarrow
%% inv.\phi$, where $inv.pred$ is a predicate for the set of states and
%% $inv.\phi$ is a condition providing a witness for the agents which
%% must be enabled when $pred$ holds. Typically, $inv.\phi$ is either
%% $\forall i: \g(i)$ or $\g(\ptr)$, where $\g(i)$ is the disjunction of
%% $\g(fl(i))$ for all flows $fl$ of the protocol, and $\ptr$ is some
%% protocol variable with values in $\IndexSet$.

%% \Fig{figSpecGenDetails} presents the overview of our method for
%% generating the set of invariants $\InvSet$ by iteratively adding
%% witness variables. As shown in the figure, our method starts with an
%% initial set of invariants, $\InvSet$ $=$ $\{true$ $\rightarrow$
%% $\forall i: \g(i)\}$. Next, the set of invariants, $\InvSet$, is
%% iteratively verified to refine the set of invariants in $\InvSet$. The
%% verification is done by model checking a protocol model with a small
%% number of ($c$) agents: as a heuristic this number is one more than
%% the maximum number of agents involved in the guard and action of the
%% rules of the flows of the protocol. Thus, for the German protocol
%% example, $c$ is 2.
%% }

%% \begin{figure}
%% \includegraphics[scale=.5]{./Figures/progressSpecGenDetails.jpg}
%% \caption{Method Overview}
%% \label{figSpecGenDetails}
%% \end{figure}

%% [TBD PLEASE]

%% If the model checking fails for some invariant $inv \in InvSet$, the
%% returned counterexample is inspected by the user. The failure of $inv$
%% occurs due to some agent $i$ which should have had some flow enabled
%% according to $inv$ but does not. This can have two causes: (1) there
%% is a bug in either the flow or the protocol code and thus the flow is
%% not enabled, or (2) the predicate of the invariant $inv$ is too
%% weak---the flow $i$ cannot be enabled in some state included in the
%% predicate due to another agent $j$ whose flow is enabled and must
%% update the state. We refer to this case by saying that the flow of
%% agent $i$ is in {\em conflict} with flow of agent $j$.

%% In case of a conflict, the invariant is split to accommodate the
%% conflicting agent by: (1) finding a witness variable $\ptr$ in the
%% protocol which points to $j$ and (2) finding a conflict condition
%% $conf$ which must hold when the conflict happens. Then, as shown in
%% \Fig{fig:SplitMethod}, the invariant $inv$ is split to $inv1$ and
%% $inv2$: $inv1$ essentially strengthens the predicate of $inv$ with
%% $\lnot conf$ to remove the conflicting trace, and $inv2$ handles the
%% conflicting case by checking for $\g(\ptr)$ when $conf$ holds. In order
%% to ensure that $\ptr$ is not $null$ when $inv2$ holds, we require that
%% $conf \rightarrow \lnot(\ptr=null)$.

%% \input{splitMethod.tex}

%% \nop{
%% \Fig{fig:deadlockSpecGeneration} shows the specification generation as
%% a pseudo-code which explains how the invariant is split to refine the
%% skolemization. The key rationale behind the splitting is to: (1)
%% ensure that the preconditions of the new invariants add up to the
%% precondition of the invariant split, and (2) the right hand side must
%% imply that some flow of at least one agent is enabled. Thus it is
%% either $\forall i: \g(i)$, i.e. all agents have some flow enabled, or
%% it says that some flow of agent $\ptr$ is enabled, i.e. $\g(\ptr)$ where
%% $\ptr$ is ensured to be non-null by the precondition $pre$.
%% }

%% \nop{ present a method for deriving flow properties which can be used
%%   to prove deadlock freedom. The key insight behind our approach is
%%   that in a deadlock state, all flows must be blocked[define]. Thus,
%%   to prove deadlock freedom, we need to show that at all times, some
%%   flow is enabled.  }

%% \nop{
%% %\subsection{Flow enabled property}
%% as described in \Fig{figExperimentalSetup} Continuing on the 

%% The flow enabled property states that 'at all times, {\em some} flow
%% must be enabled'. The usage of some introduces an existential
%% quantification: this is eliminated by iterative skolemization, i.e.,
%% iterative addition of information about which flow can make progress
%% at a particular state. This is done by starting with an initial
%% specification $G(\exists i: enb(i)$ and generating invariants of the
%% form $G(enb(f(s_G)))$ by iterative skolemization. This is accomplished
%% by starting with an initial guess of $f$ to be true and iteratively
%% splitting $f$ based on counterexamples, as illustrated by the
%% pseudo-code shown in \Fig{fig:deadlockSpecGeneration}.

%% \input{methodPseudocode.tex}
%% }

%% }

%\subsection{German Protocol}
\subsection{Specifying Invariants for the German Protocol}
\label{sec:GermanInvariantGeneration}
We now describe the complete generation of the invariants for the
German protocol. We start with the initial invariant that for all
agents, some flow is enabled. This can be stated as: \[true
\rightarrow \forall i \in \IndexSet \, \g(i)\tag{inv-1}.\]
%Continuing on our example of the German protocol, the flow enabled
%property can initially be skolemized to hold for all $i$:
\nop{
\begin{equation}
\forall i:\g(i), \tag{inv-1}\label{inv1}
\end{equation}
}
%where, $\g(i)$ $=$ $\g(\Shared(i))$ $\lor$ $\g({\Exclusive}(i))$ $\lor
%\g(\Invalidate(i))$. 
%e invariant
%that all flows can make progress for all caches $i$.

This invariant fails on model checking with 3 caches.  A
counterexample is returned in which the \Exclusive flow of cache 1 was
expected to be enabled but is not since the \Exclusive flow of cache 2
is being processed, i.e., the pointer $CurPtr$ points to 2. Thus, on
inspecting the guard of the disabled rule ($RecvReqE$) of the
\Exclusive flow, the invariant is split by selecting the witness
variable $\ptr$ to be $CurPtr$ and the conflict condition $conf$ as
$\lnot(CurCmd=Empty)$. The generated invariants are:

\begin{enumerate}
\item The first invariant states that when $CurPtr$ is $null$, all
  flows of all caches are enabled. This is specified as:
  \[(CurCmd=Empty) \rightarrow \forall i \in \IndexSet \, \g(i)\tag{inv-1.1}.\]

\item The second invariant states that when $CurPtr$ is not $null$,
  the agent pointed to by $CurPtr$ must have some flow enabled. This
  can be stated as \(\lnot(CurPtr=null) \rightarrow \g(CurPtr)\). In
  order to bring it in the quantified invariant form, we write it
  as: \[\lnot(CurCmd=Empty) \rightarrow \forall i \in \ISet{inv-1.2}
  \, \g(i)\tag{inv-1.2},\] where $\ISet{inv-1.2} = {i:(i \in
    \IndexSet)\land(i=CurPtr)}$. Also, the an assertion checking
  $\lnot (CurCmd=Empty) \rightarrow \lnot (CurPtr=null)$ is added.
\end{enumerate}

\nop{
\begin{equation}
(CurPtr=NULL) \rightarrow \forall i: enb(i)\tag{inv-1.1}\label{inv11}
\end{equation}

\begin{equation}
\lnot(CurPtr=NULL) \rightarrow \g(CurPtr) \tag{inv-1.2}\label{inv12}
\end{equation}
}

Next, on model checking the invariants inv-1.1 and inv-1.2, the
invariant inv-1.2 fails. The counterexample trace shows that when the
\Exclusive flow is supposed to be enabled for agent 1 (i.e. when
$CurPtr=1$), it is not enabled. This is due to a conflict with the
\Invalidate flow of agent 2: the guard of the rule $SendGntE$ of the
\Exclusive flow requires all sharers to be invalidated, which is what
the enabled \Invalidate of agent 2 is doing . Thus, the invariant
inv-1.2 is split by selecting the witness $\ptr$ to be an auxiliary
variable $Sharer$ which points to the last sharer added to the set of
sharers, $ShrSet$.  The conflict condition checks if some \Invalidate
needs to be sent and is thus derived from the guard of the
$SendInvalidate$ rule and is equal to $(Inv\_Cond$ $\land$ $\lnot
(Sharer=null))$ [CHECK ME]. The two invariants thus obtained are:

\begin{enumerate}
\item The first invariant says that when an \Invalidate is not
  required, some flow of agent pointed to by $CurPtr$ is enabled:
  \[\lnot(CurCmd=Empty) \land (\lnot Inv\_Cond) \rightarrow \forall i \in \ISet{inv-1.2.1} \, \g(i)\tag{inv-1.2.1},\] 
where \ISet{inv-1.2.1} = \ISet{inv-1.2}.

\item The second invariant states that if the condition for
  \Invalidate is $true$ (i.e. $Inv\_Cond$ $true$) and there is a
  sharer (i.e. $Sharer$ is not $null$), then some flow for agent
  pointed by $Sharer$ must be $true$. This is stated as:
  \[\lnot(CurCmd=Empty) \land (Inv\_Cond) \rightarrow \forall i \in
  \ISet{inv-1.2.2} \, \g(i)\tag{inv-1.2.2},\] where $\ISet{inv-1.2.2}
  = \{i|(i \in \IndexSet)\land(i \in ShrSet)\}$.
\end{enumerate}

Next, on model checking, the invariants inv1-1, inv-1.2.1, inv-1.2.2
hold for a model with 3 caches. Then, this set of invariants form a
candidate set to verify for a protcol model with an unbounded number
of agents, in order to proves \mdeadlock freedom. The property is
checked for unbounded agents using techniques described in
\Sec{sec:CMP}.

\subsection{Proof of soundness}
We show that the invariants in \InvSet generated using our method,
collectively imply \mdeadlock freedom. We show this by first stating
the following lemma (proof in Appendix~\ref{sec:proof}):

\newtheorem*{lem1}{Lemma}
\begin{lem1}
The following condition holds for \InvSet: $\bigvee_{inv \in \InvSet}
inv.pred = true$.
\end{lem1}

%% \nop{
%% All the invariants
%% in \InvSet have the form $pred \rightarrow \phi$, where, $pred$ is a
%% predicate, and $\phi$ is either $\forall i: \g(i)$ or is $\g(\ptr)$,
%% for some variable $\ptr$ such that $pred \rightarrow
%% \lnot(\ptr=null)$. And (2), the predicates of all the invariants in
%% \InvSet add up to true, i.e., $\bigvee_{inv \in \InvSet} inv.pred =
%% true$.
%% \end{lem1}}

%% \nop{
%% \begin{proof}
%% We prove this by induction over the splitting steps in our method.

%% {\em Base Case:} Our method starts with only the initial invariant
%% $true \rightarrow \forall i: \g(i)$ in \InvSet. Thus, it trivially
%% satisfies the lemma.

%% {\em Induction Step:} Next, suppose at some point during the
%% generation of invariants, the set of candidates is \InvSet. On model
%% checking, invariant $inv$ in \InvSet fails and is thus split by
%% calling \SplitMethod(conf, \ptr,inv), with invariants $inv1$ and
%% $inv2$ returned. Then, the new set of invariants, $\InvSet'$ $=$
%% $\InvSet$ $\setminus$ $\{inv\}$ $\cup$ $\{inv1,inv2\}$.

%% As can be seen from \Fig{fig:SplitMethod}, $inv1.\phi = inv.\phi$, and
%% further $inv1.pred \rightarrow inv.pred$. Then, in case $\phi$ is
%% $\forall i: \g(i)$, $inv1$ trivially satisfies condition (1). In case
%% $\phi$ is $\g(\ptr)$, since $inv1.pred \rightarrow inv.pred$ (from
%% \Fig{fig:SplitMethod}) and $inv.pred \rightarrow \lnot(\ptr=null)$ (by
%% assumption of the induction step), the condition $inv1.pred
%% \rightarrow \lnot(\ptr=null)$ holds. Thus, $inv1$ satisfies condition
%% (1). Next, $inv2$ is of the form $inv.pred \land conf \rightarrow
%% \g(\ptr)$. Since $conf \rightarrow \lnot(\ptr=null)$ (from
%% \Fig{fig:SplitMethod}), $inv2$ satisfies (1) as well.

%% Finally, as can be seen from \Fig{fig:SplitMethod}, the disjunction of
%% predicates $inv1$ and $inv2$ equals to the predicate of $inv$. Thus,
%% the sum of predicates of the new and old set of invariants is the
%% same, i.e., $\bigcup_{inv \in \InvSet} inv.pred$ = $\bigcup_{inv \in
%%   \InvSet'} inv.pred$. This proves (2).

%% Thus, by induction, both conditions, (1) and (2) hold. 
%% \end{proof}
%% }

Intuitively, this condition states that the predicates of all the
invariants in \InvSet add up to \true. Thus, in every state of the
protocol, $inv.pred$ holds for some $inv \in \InvSet$.  This condition
enables the proof of the following Theorem (proof in appendix).

\newtheorem*{lem3}{Theorem}
\begin{lem3}
The set of invariants $\InvSet$ collectively imply \mdeadlock freedom,
i.e., $(\forall inv \in \InvSet, \Protocol \models inv) \rightarrow
\Protocol \models (\bigvee_{i} \bigvee_{rl(i)} rl(i).\rho)$.
\end{lem3}

%% \nop{
%% \begin{proof}

%% Let the protocol be in some state $s$. We argue that some flow is
%% enabled in this state. By the above lemma, there must exist some
%% invariant, $inv$, for which the predicate holds, i.e., $inv.pred$
%% holds in $s$ (from Condition (2) of the lemma). Then, by Condition (1)
%% of the above lemma, $inv.\phi$ has either the form $\forall i: \g(i)$
%% or has the form $\g(\ptr)$, for some variable $\ptr$ such that $pred
%% \rightarrow \lnot(\ptr=null)$. In the first case, agent $0$ trivially
%% satisfies the property. In the second case, the agent pointed by
%% $\ptr$ satisfies the property: note that \ptr is not $null$ as shown
%% in lemma.

%% Then, in each reachable state of the protocol $s$, some flow must be
%% enabled. And thus, some transition must be enabled. This proves the
%% \Enabled property and \mdeadlock freedom.
%% \end{proof}
%% }


%% \nop{
%% \begin{proof}
%% We show this by showing that the set of invariants verified using the
%% model checker at all points in the loop have antecedents adding up to
%% true.

%% The initial invariant states that for all caches, some flow is
%% enabled.  Thus it trivially has at least one cache enabled, i.e.,
%% $true \rightarrow \forall i: \g(i).$

%% Now, at each point, when an invariant inv is split, the splitting is
%% done by choosing a precondition $pre$ such that:

%% Invariant 1 is $pre \land inv.pre \rightarrow \phi1$ where, $\phi1$ is
%% either $\forall i: \g(i)$, or, $phi$ is $\g(ptr1)$ for some $ptr1$
%% such that $pre1 \land inv.pre \rightarrow \lnot(ptr1=null)$, and
%% Invariant 2 is: $\lnot pre \land inv.pre \rightarrow \phi2$ where,
%% $\phi2$ is either $\forall i: \g(i)$, or, $phi2$ is $\g(ptr2)$ for
%% some $ptr2$ such that $pre2 \land inv.pre \rightarrow
%% \lnot(ptr2=null)$.

%% Clearly, the preconditions on splitting add up to the precondition of the
%% split invariant.

%% Then, by induction, the preconditions of the invariants add up to
%% true.  Thus, at all times, at least one of the invariants must have a
%% precondition true. Then, if the right hand side of the invariant is
%% $\forall i: \g(i)$, some flow corresponding to all agents is
%% enabled. Alternately, if the right side is $\g(\ptr)$ for some ptr, then
%% since $pre \rightarrow \ptr$, some flow of agent $\ptr$ must be enabled.

%% Then, by induction we have shown that some flow is always enabled and
%% thus the \Enabled property.

%% \end{proof}

%% }

%% \nop{
%% Next, we show that the \Enabled property implies deadlock freedom.

%% \newtheorem*{lem4}{Theorem 2}
%% \begin{lem4}
%% The \Enabled property implies deadlock freedom.
%% \end{lem4}

%% In the next section we show how the flow enabled property can be
%% verified for an arbitrary number of agents for a protocol.

%% \nop{
%% before the flow can
%% progress.  This can be seen from the guards of $SendGntS$ and
%% $SendGntE$---$ExGntd$ must be false and in case of $SendGntE$, the
%% ShrSet must be null. We assume that the one of the caches in the
%% ShrSet is pointed by $cache\_inv$ (implemented as an auxiliary
%% variable) and that $cache\_inv$ is null if and only if ShrSet is
%% empty. Then, $((CurCmd=ReqE)|((CurCmd=ReqS) \land ExGntd)) \land
%% cache\_inv!=NULL)$ implies that invalidate must happen.


%% Progress of the request is stuck since another flow is making
%% progress at the directory. In the German protocol, in case the
%% directory is processing a request from a cache, it points to the cache
%% through $curptr$. Thus, if $curptr!=i$, $progress(i)$ will fail for
%% cache $i$. This can be seen from the guard of $SendGntS(i)$ and
%% $SendGntE(i)$ in protocol code---the guard requires $curptr=i$. Thus,
%% the user can strengthen the property by splitting the
%% invariant~\ref{inv1} into two as follows:


%% The progress invariants are first generated by iteratively model
%% checking a model with 2-3 caches. After generation, these invariants
%% are then checked for an unbounded number of caches.

%% The generation is done using 2-3 caches because of two factors: (1) a
%% smaller model is easy to iterate model checking on and, (2) progress
%% proof from smaller model typically generalizes to unbounded number of
%% caches---a consequence of the fact that protocol designers think in
%% terms of a small number of caches. 

%% The generation is done as follows:

%% (1) First, the user adds invariants for progress of flow corresponding
%% to each request. Thus, the invariant 

%% \begin{equation}
%% \forall i:progress(i), \tag{inv-1}\label{inv1}
%% \end{equation}

%% where, $progress(i) = (progress(\Shared(i))|progress(\Exclusive(i)))$,
%% is added.

%% (2) Second, model checking is done on this. If the model checking
%% succeeds, progress is proven. 

%% (3) If the model checking fails, as happens in this case, the user
%% inspects the counter-example. The following situations can create the
%% counter-example:

%% a) Progress of the request is stuck since another flow is making
%% progress at the directory. In the German protocol, in case the
%% directory is processing a request from a cache, it points to the cache
%% through $curptr$. Thus, if $curptr!=i$, $progress(i)$ will fail for
%% cache $i$. This can be seen from the guard of $SendGntS(i)$ and
%% $SendGntE(i)$ in protocol code---the guard requires $curptr=i$. Thus,
%% the user can strengthen the property by splitting the
%% invariant~\ref{inv1} into two as follows:

%% \begin{equation}
%% (curptr=NULL) \rightarrow \forall i: progress(i)\tag{inv-1.1}\label{inv11}
%% \end{equation}

%% \begin{equation}
%% \forall i:(curptr=i) \rightarrow progress(i) \tag{inv-1.2}\label{inv12}
%% \end{equation}

%% %$curptr=NULL \rightarrow \forall i: progress(i)$ and $\forall i:
%% %curptr=i \rightarrow progress(i)$.

%% Note that the disjunction of antecedents of the above two invariants
%% is $true$. This is required to prove progress in all cases.

%% b) Next, even after the above strengthening, the invariants fail. This
%% is because an invalidate may be required before the flow can progress.
%% This can be seen from the guards of $SendGntS$ and
%% $SendGntE$---$ExGntd$ must be false and in case of $SendGntE$, the
%% ShrSet must be null. We assume that the one of the caches in the
%% ShrSet is pointed by $cache\_inv$ (implemented as an auxiliary
%% variable) and that $cache\_inv$ is null if and only if ShrSet is
%% empty. Then, $((CurCmd=ReqE)|((CurCmd=ReqS) \land ExGntd)) \land
%% cache\_inv!=NULL)$ implies that invalidate must happen.

%% Thus invariant~\ref{inv12} can be split into two invariants as
%% follows:

%% \begin{equation}
%% \forall i:(curptr=i) \land !(Inv\_Cond \land
%% cache\_inv=NULL)\rightarrow progress(i)\tag{inv-1.2.1}\label{inv121}
%% \end{equation}

%% %$\forall i:(curptr=i) \land !(Inv\_Cond \land
%% %cache\_inv=NULL)\rightarrow progress(i)$
%% %
%% %and

%% \begin{equation}
%% \forall i,j: (curptr=i) \land Inv\_Cond \land (j= cache\_inv)
%% \rightarrow progress\_invalidate(j),\tag{inv-1.2.2}\label{inv122}
%% \end{equation}

%% %$\forall i,j: (curptr=i) \land Inv\_Cond \land (j= cache\_inv)
%% %\rightarrow progress\_invalidate(j)$,

%% where, $Inv\_Cond$ is $((CurCmd=ReqE)|((CurCmd=ReqS) \land ExGntd))$.

%% %and the value of $cache\_inv$ dictate if the
%% %invalidate flow is fired.  The $Inv\_Cond$ condition checks if (1)
%% %current request is Exclusive $(CurCmd=ReqE)$, or, (2) Current request
%% %is shared and there is some other cache with exclusive
%% %$(CurCmd=ReqS) \land ExGntd)$. Thus, $Inv\_Cond$ =
%% %$((CurCmd=ReqE)|((CurCmd=ReqS) \land ExGntd))$. Finally, the $cache\_inv$ is
%% %an auxiliary variable which points to one of the caches which need to
%% %be invalidated, it is $NULL$ if no cache needs to be invalidated.

%% For the German protocol, \ref{inv11}, \ref{inv121}, \ref{inv122} are
%% invariants.
%% }
%% \nop{
%% The following situations can create the counter-example: a) Progress
%% of a request is stuck due to a conflicting flow (directory
%% pending). The information of this conflicting flow is typically stored
%% in the directory or can be added as an auxiliary variable. (b) Waiting
%% for another flow to complete -- for example invalidates. In this case,
%% the directory again stores information about the flow it is waiting
%% for. And thus, information is added by the user accordingly.
%% }



%% \nop{

%% \subsection{Progress from Flows}
%% Progress can be defined for each flow as a logical or of the guards of
%% all contained rules. We denote this as $Progress_{fl}(i,j)$ for flow
%% $fl$ to make progress on caches $i,j$. In case one of many flows can
%% make progress for these caches, we write progress as
%% $Progress_{fl1,fl2,\ldots,fln}(i,j)$ to denote that $fl1$ or $fl2$ or
%% $fl3$ $\ldots$ $fln$ can make progress. Finally, we define
%% $Progress(i,j)$ as the logical or of progress of all flows: i.e. any
%% flow can make progress on $(i,j)$.

%% \subsection{Generating Specification}
%% The pseudo-code for generating deadlock specification is shown in
%% \Fig{fig:deadlockSpecGeneration}.

%% \input{methodPseudocode.tex}
%% }

%% \nop{
%% Invariant set, $\mathcal{I}$: \{$\forall(i,j):$ $G \rightarrow
%% Progress(i,j)$\}, where $G=true$ and
%% $Progress(i,j)=Progress(fl_1(i,j)) \lor Progress(fl_2(i,j))\ldots \lor
%% Progress(fl_n(i,j))$.
%% %where  i.e. for all pairs $i$
%% %and $j$, some flow $fl(i,j)$ can make progress.

%% 1) Model check for all invariants in $\mathcal{I}$. 

%% If any invariant $inv \in \mathcal{I}$ is false, goto 2. Else goto 3.
%% Note that $inv$ is of the form $\forall i,j: G_I \rightarrow \phi$.

%% 2) When $inv$ fails, a counter-example is found. This counter-example
%% restricts that progress can only occur if $i$ and $j$ specify some
%% guard. Thus, $inv$ can be split as:

%% %$\forall(i,j) pred_1(i,j):Progress(i,j)$ and $\forall(i,j)
%% %pred_2(i,j):Progress(i,j)$, 

%% $\forall i,j: G_I \land pred_1 \rightarrow \phi$ and $\forall i,j: G_I
%% \land pred_2 \rightarrow \phi$, where, $pred_1 \lor pred_2 = true$ and
%% $pred_1 \land pred_2 = false$.

%% Update $\mathcal{I}$ and go back to step 1.

%% 3) Once all invariants in $\mathcal{I}$ hold, we have proven progress.
%% }

%% \nop{
%% \newtheorem*{lem1}{Theorem}
%% \begin{lem1}
%% If the invariants in $\mathcal{I}$ hold, progress is proven.
%% \end{lem1}

%% \begin{proof}
%% The invariants in $\mathcal{I}$ are of the form: $\forall(i,j)
%% pred_m(i,j):Progress(i,j)$, for $m \in \{1 \ldots r\}$, where the or
%% of all $pred_s$ is true and all the pairs $(pred_r,pred_s)$ are
%% disjoint (i.e. $pred_r \land pred_s = false$).

%% Then, since at all times, exactly one $pred_s$ must hold, and since
%% $\forall(i,j) pred_s(i,j):Progress(i,j)$ holds, $Progress(i_s,j_s)$ is
%% true since $pred_s$ holds. Hence the protocol can make progress. Hence
%% proved.

%% \end{proof}
%% }
%% }


==> germanCode.tex <==

\begin{figure}
\begin{minipage}{\textwidth}
\begin{minipage}[h]{\textwidth}
        \Ruleset{$\forall i \in \Caches:$}{SendReqS}{$(Chan1[i].Cmd = Empty) \land \Caches[i].State = I$}{$Chan1[i].Cmd := ReqS$;} 
        \Ruleset{$\forall i \in \Caches:$}{RecvReqS}{$(\curcmd = Empty) \land Chan1[i].Cmd = ReqS$}{$\curcmd := ReqS$; $\curptr := i$; 

$Chan1[i].Cmd := Empty$; $for \; j: \Caches do InvSet[j] := ShrSet[j] \; end;$}       


%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 2$ $\wedge$ 

%% $p_0[i].lock=0$}{$p_0[i].lock := i$;

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 3$}{$p_1[i]$ $:=$ $p_0[i].next$;

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 4$ $\wedge$ 

%% $p_1[i].lock=0$}{$p_1[i].lock := i$;

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 5$}{$if(p_1[i].key<Key)$;

%%  \hspace*{3mm} $pc[i]++;$

%%  \hspace*{3mm} $else$ $pc[i]=10;$

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 6$}{$p_0[i].lock := 0$;

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 7$}{$p_0[i]$ $:=$ $p_1[i]$;

%%  \hspace*{3mm} $pc[i]++;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 8$}{$p_1[i]$ $:=$ $p_0[i].next$;

%%  \hspace*{3mm} $pc[i]++;$} 

%% \end{minipage} \hspace{1em} 
%% \hfill
%% \begin{minipage}[h]{.45\textwidth}
%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 9$ $\wedge$ 

%% $p_0[i].lock=0$}{$p_1[i].lock := i$;

%%  \hspace*{3mm} $pc[i] := 5;$} 

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 10$}{if $(p_1[i].key = Key)$ 

%%  \hspace*{3mm} then $pc[i]++;$ 

%%  \hspace*{3mm} else $pc[i]=15;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 11$}{$p_2[i]$ $:=$ $p_1[i].next;$ $pc[i]++;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 12$}{$p_0[i].next$ $:=$ $p_2[i];$ $pc[i]++;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 13$}{$result[i]$ $:=$ $true;$

%% \hspace*{3mm} $pc[i]$ $:=$ $pc[i]+3;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 14$}{[else] $pc[i]++;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 15$}{$result[i]$ $:=$ $false;$ $pc[i]++;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 16$}{$p_0[i].lock := 0;$ $pc[i]++;$}

%%         \RulesetSh{$\forall i \in \Threads:$}{$pc[i] = 17$}{$p_1[i].lock := 0;$}

\end{minipage} \hspace{1em} 
\captionof{figure}{Murphi model for method $\Remove$ for thread \(i\): each rule corresponds to a line
in the $\Remove$ method shown in \Fig{fig:remove}. \label{fig:RemoveMurphi}}
\end{minipage}
\caption{German code}
\label{figGermanCode}
\end{figure}


==> methodPseudocode.tex <==
\begin{figure}
\centering
\begin{minipage}[b]{\textwidth}
%    \begin{minipage}{\textwidth}
{\sc generateDeadlockSpecification($\Protocol(c)$):}
      \begin{algorithmic}        
         \IndState[0]{$\InvSet = \{true \rightarrow \forall i: g(i)\}$}
         \IndState[0]{while($\exists inv \in \InvSet: inv \not\models P$)}
         \IndState[1]{User inspects counterexample:}
         \IndState[1]{If real:} 
         \IndState[2]{Real bug found; Exit;}
         \IndState[1]{If spurious:}
         \IndState[2]{$(inv1,inv2)$ = \SplitMethod$(inv)$}
         \IndState[2]{$\InvSet = ((\InvSet \cup \{inv1,inv2\}) \setminus inv)$}
         \IndState[0]{return \InvSet}
      \end{algorithmic}
%    \end{minipage}
\end{minipage} \hspace{1em} 

\begin{minipage}[b]{\textwidth}
%    \begin{minipage}{\textwidth}
 \SplitMethod$(inv)$:
      \begin{algorithmic}        
        \IndState[0]{Let $inv = inv.pre \rightarrow \phi$}
        \IndState[0]{Inspect counterexample and let:} 
        \IndState[1]{Variable $ptr$: $ptr \in \IndexSet$, and}
        \IndState[2]{$a_{ptr}$ conflicts with $inv$}
        \IndState[1]{Precondition $pre$ such that:}
        \IndState[2]{Conflict happens when $pre$ holds, and}
        \IndState[3]{$pre \rightarrow \lnot(ptr=null)$}
        \IndState[1]{$inv1: \lnot pre \land inv.pre \rightarrow \phi$} 
        \IndState[1]{$inv2: pre \land inv.pre \rightarrow g(ptr)$}
        \IndState[0]{return $(inv1,inv2)$}
      \end{algorithmic}
%    \end{minipage}
\end{minipage} \hspace{1em} 

\caption{Generating Deadlock Specification}
\label{fig:deadlockSpecGeneration}
\end{figure}


==> related_Murali.tex <==
\subsection{Related Work}
\label{sec:related}

Parameterized verification, mainly of cache coherence
and mutual exclusion protocols, has received considerable
attention.  Recent methods have been based on
invisible invariants~\cite{AronsRuah:01}, 
counter abstraction~\cite{Pnuelixu},
indexed predicates~\cite{Lahiri:04a}, 
ordinary model checking~\cite{Abdullah:99a}, 
WS1S ~\cite{Baukus:02a}, learning~\cite{Grinchtein:06},
strengthening split invariants~\cite{Cohen:07}, 
and environment abstraction~\cite{Self:06,Self:08}. 
These techniques have had varying degrees of success, 
but none of them has been
applied to a large industrial-strength protocol like Flash
(although environment abstraction~\cite{Self:08} has been applied to a
simplified version of Flash).

McMillan introduced the CMP method 
in a series of papers~\cite{McMillan:Toma,McMillan:Flash,CMP}
(the proof in~\cite{McMillan:Flash} does not
completely follow the CMP framework: to get BDDs to scale, the Flash model
had to be pruned by hand.) 
Chou, Mannava, and Park~\cite{CMP} elaborated on the method
and showed how it can be performed in conjunction with any model
checker. Krstic~\cite{Krstic:AVIS} gave a formalization of the method.

As far as we are aware, the CMP method is one of the few methods to handle
the full complexity of the Flash protocol.  A transaction-based
method~\cite{ParkDill:96} and a predicate abstraction-based
method~\cite{DasDill:99} have both verified the safety properties of Flash.
Both the methods required extensive manual guidance and took several days to
complete the verification.  Recently, some nearly automatic methods based on
BDDs have been proposed~\cite{LvYi:2007,Bingham:2008}.  As with the other
BDD-based methods~\cite{McMillan:Flash}, they have trouble scaling up: they
have been able to verify only a control property, but not data.  For all of
these methods applied to Flash, model checking has taken roughly a couple
hours.  In contrast, our work is able to check both the data and control
properties of Flash in just 120 seconds. 

We note that our method of deriving
invariants from message flows is not specific to CMP, and can potentially be
used in conjunction with any other method of protocol verification.

Finally, the compositional reasoning principle at the heart of our new
analysis of CMP is similar to principles proposed by Abadi and
Lamport~\cite{AbadiLamp:93,AbadiLamp:95}, McMillan~\cite{McMillan:Toma},
Krstic~\cite{Krstic:AVIS}, Bhattacharya et al.~\cite{Ritwik} and Chen et
al.~\cite{ChenGanesh:07}.

We introduce preliminary concepts in Section~\ref{sec:prelim},
derive protocols invariants from message flows in Section~\ref{sec:flows},
present a new analysis of CMP in Section~\ref{sec:cleancmp},
show how to use flow-derived invariants with CMP in Section~\ref{sec:augcmp},
give experimental results in Section~\ref{sec:results},
and conclude with Section~\ref{sec:conclusion}.


==> splitMethodBackup.tex <==
\begin{figure}
%\centering
\begin{minipage}[b]{\textwidth}
\footnotesize
%    \begin{minipage}{\textwidth}
 {\sc Derive\_Invariants(\Protocol(c))}:
      \begin{algorithmic}[1]        
        \IndState[0]{$\InvSet = \{ \true \Rightarrow \big(\forall i \in \IndexSet: \, \g(\AgentRuleSet(i))\big)\}$}
        \IndState[0]{$\AssertSet = \{\}$}
        \IndState[0]{while $\Protocol(c) \not\models \InvSet$ do}
        \IndState[0.5]{Let $inv \in \InvSet: \Protocol(c) \not\models inv$ and

                      $inv:$ $inv.pred \Rightarrow \big(\forall i \in \ISet{inv}: \g(\AgentRuleSet(i))\big)$, where, $\ISet{inv} \subseteq \IndexSet$} 
%        \IndState[1]{$inv = inv.pred \Rightarrow \big(\forall i \in \ISet{inv}: \g(\AgentRuleSet(i))\big)$, where, $\ISet{inv} \subseteq \IndexSet$} 
%        \IndState[0.5]{User inspects $cex: s_0 \rightarrow^{\tau_0} \rightarrow^{\tau_1} \rightarrow^{\tau_2} \ldots \rightarrow^{\tau_{v-1}} s_v$ and identifies:}
        \IndState[0.5]{From $cex$ and failing state $s_f$, identify conflicting agents $i_f$ and $i_s$ s.t.}
        \IndState[1]{(1) $i_f: \big((i_f \in \ISet{inv}) \land (\lnot \g(\AgentRuleSet(i_f))\big)$ holds in $s_f$.}
        \IndState[1]{(2) $\exists rl_j \in \flow(i_f)$ s.t. $(\precon{\flow}{rl_j}{i_f} \land \lnot(\g(\flow(i_f))$ holds in $s_f$.}
        \IndState[1]{(3) $\big(i_s \not\in \ISet{inv} \land \g(\AgentRuleSet(i_s)\big)$ holds in $s_f$.}
        \IndState[0.5]{Identify $conf$ and witness $\ptr$ from above information}
%s.t. $(conf \Rightarrow \lnot rl.\rho)$ in $s_v$}
%        \IndState[0.5]{Identify variable $\ptr$ s.t. $(\ptr=i_s)$ in $s_v$}
        \IndState[0.5]{$inv1:$ $(\lnot conf \land inv.pred) \Rightarrow \big(\forall i \in \ISet{inv}: \, \g(\AgentRuleSet(i)\big)$} 
        \IndState[0.5]{$inv2:$ $(conf \land inv.pred) \Rightarrow \big(\forall i \in \ISet{inv2}: \, \g(\AgentRuleSet(i)\big)$, where,
%        \IndState[1]{$\ISet{inv2} = \{i| \, i = \ptr\}$} 

                       $\ISet{inv2} = \{i| \, i = \ptr\}$}
        \IndState[0.5]{$\InvSet = \{\InvSet \setminus inv\} \cup \{inv1,inv2\}$}
        \IndState[0.5]{$\AssertSet = (\AssertSet \setminus \big(inv.pred \Rightarrow (\ISet{inv} \neq \{\})\big) \; \cup$ 

                       $\{\big(inv1.pred \Rightarrow (\ISet{inv1} \neq \{\})\big),\big(inv2.pred \Rightarrow (\ISet{inv2} \neq \{\})\big)\}$}
%        \IndState[0.5]{$\AssertSet = \AssertSet \cup \{(inv1.pred \rightarrow \ISet{inv1}),(inv2.pred \rightarrow \ISet{inv2})\}$}
      \end{algorithmic}
%    \end{minipage}
\end{minipage} \hspace{-5em} 
\caption{Method for Deriving Invariants from Flows.}
\label{fig:MethodOverview}
\end{figure}


\nop{
\begin{figure}
%\centering
\begin{minipage}[b]{\textwidth}
\footnotesize
%    \begin{minipage}{\textwidth}
 Generate\_Invariant(P(c)):
      \begin{algorithmic}[1]        
        \IndState[0]{$\InvSet = \{ \forall i \in \IndexSet: \g(i)\}$}
        \IndState[0]{while $P(c) \not\models \InvSet$ do}
        \IndState[0.5]{Let $inv \in \InvSet$: $P(c) \not\models inv$, s.t.,} 
        \IndState[1]{$inv: inv.pred \rightarrow \forall i \in \IndexSet^{inv} \g(i)$, where, $\IndexSet^{inv} \subseteq \IndexSet$} 
%        \IndState[1]{Case 1: Let $inv: pred \rightarrow \forall i \g(i)$:}       
%        \IndState[2]{Let $i_s$ be such that $\g(i_s) \not\models P(c)$}
%        \IndState[1]{Case 2: Let $inv: pred \rightarrow \g(i_0)$:}
%        \IndState[2]{Let $i_s = i_0$, clearly, $\g(i_s) \not\models P(c)$}
        \IndState[0.5]{User inspects $cex: s_0 \rightarrow^{\tau_0} \rightarrow^{\tau_1} \rightarrow^{\tau_2} \ldots \rightarrow^{\tau_{v-1}} s_v$.}
        \IndState[1]{Case 1: discrepancy between $cex$ and flows}
        \IndState[1.5]{Fix protocol or flows}
        \IndState[1.5]{return $null$}
        \IndState[1]{Case 2: conflicting flows}
        \IndState[1.5]{The user identifies:}
        \IndState[2]{(1) $i_s: i_s \in \IndexSet^{inv} \land \g(i_s)$ is false in $s_v$}
        \IndState[2]{(2) A blocked flow $fl:$, i.e. $pre(fl(i_s)) \land \lnot(\g(fl(i_s)))$ holds in $s_v$}
        \IndState[2]{(3) Another flow $fl'$, agent $\ptr$ and condition $conf$ s.t.:}
        \IndState[2.5]{$\ptr \not\in \IndexSet^{inv} \land \g(\ptr)$ is true in $s_v$}
        \IndState[2.5]{$conf$ over-approximates the state $s_v$, in which $fl$ is blocked due to $fl'$}
        \IndState[1.5]{inv1: $\lnot conf \land inv.pred \rightarrow \forall i \in \IndexSet^{inv} \g(i)$} 
        \IndState[1.5]{inv2: $conf \land inv.pred \rightarrow \forall i s.t. i = \ptr: \g(\ptr)$}
        \IndState[1.5]{$\InvSet = \{\InvSet \setminus inv\} \cup \{inv1,inv2\}$}
        \IndState[0]{return $\InvSet$}
      \end{algorithmic}
%    \end{minipage}
\end{minipage} \hspace{-5em} 
\caption{Method Overview.}
\label{fig:MethodOverview}
\end{figure}
}

\nop{
\begin{figure}
\centering
\begin{minipage}[b]{.45\textwidth}
\footnotesize
%    \begin{minipage}{\textwidth}
 \SplitMethod(inv, \ptr, conf):
      \begin{algorithmic}        
        \IndState[0]{assert conf $\rightarrow$ $\lnot$(\ptr=null)}
        \IndState[0]{let inv = inv.pred $\rightarrow$ inv.$\phi$}
        \IndState[0]{inv1: $\lnot$ conf $\land$ inv.pred $\rightarrow$ inv.$\phi$} 
        \IndState[0]{inv2: conf $\land$ inv.pred $\rightarrow$ \g(\ptr)}
        \IndState[0]{return (inv1,inv2)}
      \end{algorithmic}
%    \end{minipage}
\end{minipage} \hspace{-5em} 
\caption{Method for splitting invariants.}
\label{fig:SplitMethod}
\end{figure}
}

